Learning from Shader Program Traces

Deep learning for image processing typically treats input imagery as pixels in some color space. This paper proposes instead to learn from program traces of procedural fragment shaders -- programs that generate images. At each pixel, we collect the intermediate values computed at program execution, and these data form the input to the learned model. We investigate this learning task for a variety of applications: our model can learn to predict a low-noise output image from shader programs that exhibit sampling noise; this model can also learn from a simplified shader program that approximates the reference solution with less computation, as well as learn the output of postprocessing filters like defocus blur and edge-aware sharpening. Finally we show that the idea of learning from program traces can even be applied to non-imagery simulations of flocks of boids. Our experiments on a variety of shaders show quantitatively and qualitatively that models learned from program traces outperform baseline models learned from RGB color augmented with hand-picked shader-specific features like normals, depth, and diffuse and specular color.

==> 9-notes.tex <==
\clearpage

\Yuting{Notes only, it's not part of the appendix.}

\section{P value on trace contubution hypothesis}

Null hypothesis:

\begin{equation}
    Pr[err_{good} \leq err_{subsample}] = \frac{1}{2}
\end{equation}

\begin{equation}
    Pr[err_{subsample} \leq err_{bad}] = \frac{1}{2}
\end{equation}

\subsection{Treat good < subsample < bad as one event}

\begin{equation}
    \begin{split}
        & Pr[err_{good} < err_{subsample} < err_{bad}] \\
        = & Pr[err_{good} \leq err_{subsample}] \cdot Pr[err_{subsample} \leq err_{bad}] \\
        = & \frac{1}{4}
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        & Pr[\text{other ordering}] \\
        = & 1 - Pr[err_{good} < err_{subsample} < err_{bad}] \\
        = & \frac{3}{4}
    \end{split}
\end{equation}

\subsubsection{All data points}

\begin{equation}
    \begin{split}
        & Pr[\text{other ordering happens at most 5 times out of 20}] \\
        = & \binom{20}{5} \cdot (\frac{3}{4})^5 \cdot (\frac{1}{4})^{15} \\
        + & \binom{20}{4} \cdot (\frac{3}{4})^4 \cdot (\frac{1}{4})^{16} \\
        + & \binom{20}{3} \cdot (\frac{3}{4})^3 \cdot (\frac{1}{4})^{17} \\
        + & \binom{20}{2} \cdot (\frac{3}{4})^2 \cdot (\frac{1}{4})^{18} \\
        + & \binom{20}{1} \cdot (\frac{3}{4})^1 \cdot (\frac{1}{4})^{19} \\
        + & \binom{20}{0} \cdot (\frac{1}{4})^{20} \\
        = & 3.8e-6
    \end{split}
\end{equation}

\subsubsection{Only one quater and one eighth}

\begin{equation}
    \begin{split}
        & Pr[\text{other ordering happens at most 0 times out of 8}] \\
        = & \binom{8}{0} \cdot (\frac{1}{4}) ^ 8 \\
        = & 1.5e-5
    \end{split}
\end{equation}

\subsubsection{Add bricks data at one quater}

\begin{equation}
    \begin{split}
        & Pr[\text{other ordering happens at most 1 times out of 9}] \\
        = & \binom{9}{1} \cdot (\frac{1}{4}) ^ 8 \cdot (\frac{3}{4})^1 \\
        + & \binom{9}{0} \cdot (\frac{1}{4}) ^ 9 \\
        = & 1.1e-4
    \end{split}
\end{equation}

\subsection{Treat good < subsample and subsample < bad independently}

\subsubsection{All data points}

\begin{equation}
    \begin{split}
        & Pr[(good > subsample) \text{ happens at most 3 times out of 20}] \\
        = & \binom{20}{3} \cdot (\frac{1}{2}) ^ 3 \cdot (\frac{1}{2})^{17} \\
        + & \binom{20}{2} \cdot (\frac{1}{2}) ^ 2 \cdot (\frac{1}{2})^{18} \\
        + & \binom{20}{1} \cdot (\frac{1}{2}) ^ 1 \cdot (\frac{1}{2})^{19} \\
        + & \binom{20}{0} \cdot (\frac{1}{2}) ^ 0 \cdot (\frac{1}{2})^{20} \\
        = & 0.00129
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        & Pr[(subsample > bad) \text{ happens at most 2 times out of 20}] \\
        = & \binom{20}{2} \cdot (\frac{1}{2}) ^ 2 \cdot (\frac{1}{2})^{18} \\
        + & \binom{20}{1} \cdot (\frac{1}{2}) ^ 1 \cdot (\frac{1}{2})^{19} \\
        + & \binom{20}{0} \cdot (\frac{1}{2}) ^ 0 \cdot (\frac{1}{2})^{20} \\
        = & 0.0002
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        Pr[\text{both event happens}] = 2.6e-7
    \end{split}
\end{equation}

\subsubsection{Only one quater and one eighth}

\begin{equation}
    \begin{split}
        & Pr[(good > subsample) \text{ happens at most 0 times out of 8}] \\
        = & \binom{8}{0} \cdot (\frac{1}{2})^8 \\
        = & 0.00390625
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        & Pr[(subsample > bad) \text{ happens at most 0 times out of 8}] \\
        = & \binom{8}{0} \cdot (\frac{1}{2})^8 \\
        = & 0.00390625
    \end{split}
\end{equation}

\begin{equation}
    Pr[\text{both event happens}] = 1.5e-5
\end{equation}

\subsubsection{Add bricks data at one quater}

\begin{equation}
    \begin{split}
        & Pr[(good > subsample) \text{ happens at most 1 times out of 9}] \\
        = & \binom{9}{1} \cdot (\frac{1}{2})^8 \cdot (\frac{1}{2})^9 \\
        + & \binom{9}{0} \cdot (\frac{1}{2})^9 \\
        = & 0.017578125
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        & Pr[(subsample > bad) \text{ happens at most 0 times out of 9}] \\
        = & \binom{9}{0} \cdot (\frac{1}{2})^9 \\
        = & 0.001953125
    \end{split}
\end{equation}

\begin{equation}
    Pr[\text{both event happens}] = 3.4e-5
\end{equation}

\section{Unified network: trace contribution to a certain channel in encoder's output channel}

Derived from equaiton 8 in https://arxiv.org/pdf/1611.06440.pdf

Because encoder contains only 1x1 conv, each pixel independently contributes to the output channel in the corresponding pixel position. Therefore, we could regard each pixel as an independent example (unlike in computing trace contribution for the entire network, pixels in the same feature map jointly contribute to the loss value).

We could simply use the abs value of the output channel as cost, because the taylor exapnsion will approximate the change in cost in either direction.

According to equation 8, this should be

\begin{equation}
    \text{score} = \sum_{\text{all pixels}} |\frac{\partial \mathbbm{O}}{\partial \mathbbm{I}} \mathbbm{I}|
\end{equation}

Here, both $\mathbbm{O}$ and $\mathbbm{I}$ are feature maps.

Tensorflow only allows computing the gradient of a scalar, so we have to make the following derivations.

Assume $m$ and $n$ are two distinct pixel indices in the feature map $m \neq n$. And since encoder contains only 1x1 conv, we have the following

\begin{equation}
    \frac{\partial \mathbbm{O}_m}{\partial \mathbbm{I}_n} = 0
\end{equation}

Therefore we could derive the gradient using the following scalar value

\begin{equation}
    \frac{\partial \sum_{\text{all pixels}} \mathbbm{O}_p}{\partial \mathbbm{I}_n} =  \sum_{\text{all pixels}} \frac{\partial \mathbbm{O}_p}{\partial \mathbbm{I}_n} = \frac{\partial\mathbbm{O}_n}{\partial \mathbbm{I}_n}
\end{equation}

The score for each trace can be rewritten into

\begin{equation}
    \begin{split}
        \text{score} = & \sum_{\text{all pixels}} |\frac{\partial \mathbbm{O}}{\partial \mathbbm{I}} \mathbbm{I}| \\
        = & \sum_{\text{all pixels}} |\frac{\partial \sum_{\text{all pixels}} \mathbbm{O}_p}{\partial \mathbbm{I}} \mathbbm{I}|
    \end{split}
\end{equation}

\section{Current Result}

\input{figtex/result_pool}

\ignorethis{

\Yuting{These are notes from last subsmission.}

\input{figtex/supp_denoising_table.tex}

Things we need to work on in the paper:
\begin{itemize}
\item 
Changes to how we handle branching, loops
- Clustering, every nth --- this is done in ablation experiment for Mandelbrot, should double check that we talk about it.

\item
Tiled training 
- integrate tiled rendering

\item
Postprocessing filters

\item
Y can update figures for post processing

\item
Ablation study: All, no perceptual, no L2, fewer layers, first 5, last 5, .... \Connelly{figures are updated, need to check that text is updated.}

\item
Update abstract to reflect postprocessing effects and other changes

\end{itemize}

Finished items (leaving the list so we can double check later in an editing pass):

\begin{itemize}
\item
Perceptual error --- changed loss in Sect 4.4

\item
Sigma on input

\item
Put in figure captions perceptual, L2 and perceptual --- \Connelly{Y and I think we decided not to do this}

\item
Texture experiments: one takes both branches, one zeroes out the path not taken
- branch not taken experiment

\item
Analyze features that are important \Connelly{Yuting is working on this}



%\input{figtex/result_pool.tex}

\end{itemize}

}

==> Learning from Shader Program Traces (EG format)/0-abstract.tex <==
\begin{abstract}
Deep learning for image processing typically treats input imagery as pixels in some color space. 
%
This paper proposes instead to learn from program traces of procedural fragment shaders -- programs that generate images. 
%
At each pixel, we collect the intermediate values computed at program execution, and these data form the input to the learned model. 
%
We investigate this learning task for a variety of applications: 
%
our model can learn to predict a low-noise output image from shader programs that exhibit sampling noise; 
%
this model can also learn from a simplified shader program that approximates the reference solution with less computation,
%
as well as learn the output of postprocessing filters like defocus blur and edge-aware sharpening.
%
Finally we show that the idea of learning from program traces can even be applied to non-imagery simulations of flocks of boids.
%
Our experiments on a variety of shaders show quantitatively and qualitatively that models learned from program traces outperform baseline
models learned from RGB color augmented with hand-picked shader-specific features like normals, depth, and diffuse and specular color.
%
%We also conduct a series of analyses that show certain features are important  within the trace: these coincide with intuitively important aspects of the program. 
%
%The important features can be helpful for selecting a good subset of trace features for learning, and even learning from a small subset of the trace already outperforms the baselines. We finally show that multiple shaders can be learned together with a shared denoising network and a lightweight shader-specific encoder.
%
\changedh{We also conduct a series of analyses that show certain features within the trace are more important, and even learning from a small subset of the trace outperforms the baselines.}

\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010575.10010755</concept_id>
  <concept_desc>Computer systems organization~Redundancy</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010554</concept_id>
  <concept_desc>Computer systems organization~Robotics</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>10003033.10003083.10003095</concept_id>
  <concept_desc>Networks~Network reliability</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>  
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Neural networks}
\ccsdesc[500]{Software and its engineering~Compilers}
\ccsdesc[500]{Computing methodologies~Computer graphics}
 % 100 means lower relevance

\printccsdesc

\end{abstract}

% apps: denoising, simplification, post-processing, simulation

==> Learning from Shader Program Traces (EG format)/0-macros.tex <==

%\def\ShowNotes{}   % Comment this out to remove notes
%\def\ShowColor{}   % Comment this out to render text with same color

\newcommand{\Var}{\mathrm{Var}}

\DeclareRobustCommand{\rchi}{{\mathpalette\irchi\relax}}
\newcommand{\irchi}[2]{\raisebox{\depth}{$#1\chi$}} % inner command, used by \rchi

% left bottom right top
%\newcommand{\trimmedteaser}[1]{\frame{\includegraphics[trim=2cm 7cm 20cm 3cm,clip,height=1in]{#1}}}
\newcommand{\trimmedteaser}[1]{\frame{\includegraphics[trim=6cm 3cm 6cm 2cm,clip,width=1.75in]{#1}}}

\newcommand*{\linkback}[1]{\Acrobatmenu{GoBack}{\color{black}#1}}

%\newcommand{\pagereftop}[1]{\hyperlink{page.\getpagerefnumber{#1}}{\pageref*{#1}}}
\newcommand{\linkoverview}[1]{\hyperlink{page.\getpagerefnumber{lbl:overview}}{#1}}

\newcommand*\rot{\rotatebox{90}}
\newcommand*\chechmark{\ding{51}}
\newcommand*\OK{\ding{51}}

% Use \jumplabel{labelname} for labels that we can jump to within a paragraph, to fix PDF not going to the right location
\newcommand{\jumplabel}[1]{\phantomsection\label{#1}}

\newcommand{\citem}{\vspace{-1.5ex}\item}
\newcommand{\citemarg}[1]{\vspace{-1.5ex}\item[\changed{#1}]}
%\newcommand{\citemarg}[1]{\vspace{-1.5ex}\item[#1]}

\newlength{\w}
\newlength{\h}
\newlength{\x}

\newcommand{\cfbox}[2]{%
    \colorlet{currentcolor}{.}%
    {\color{#1}%
    \fbox{\color{currentcolor}#2}}%
}

\newcommand{\ignorethis} [1] {}

\newcommand{\sectnum    } [1] {\ref{#1}}
\newcommand{\shortsect  } [1] {\S\sectnum{#1}}
\newcommand{\sect       } [1] {Section~\sectnum{#1}}
\newcommand{\sects      } [1] {Sections~\sectnum{#1}}
\newcommand{\appx       } [1] {Appendix~\sectnum{#1}}

\newcommand{\tbl}[1]{Table~\ref{#1}}

\newcommand{\fignum     } [1] {\ref{#1}}
\newcommand{\fig        } [1] {Figure~\fignum{#1}}

\newcommand{\eqnnum     } [1] {\mbox{(\ref{#1})}}
\newcommand{\eqn        } [1] {equation~\eqnnum{#1}}
\newcommand{\Eqn        } [1] {Equation~\eqnnum{#1}}

%\newcommand{\ourParagraph}[1]{\paragraph{#1}}
\newcommand{\ourParagraph}[1]{\textit{#1}}

\newcommand{\X}{$\times$\xspace}
\newcommand{\tX}{\hspace{-0.1em}$\small\times$\hspace{-0.2em}}

\newcommand{\Mod}[1]{\ (\text{mod}\ #1)}

\newcommand{\shrinkbefore}{\vspace{-0.6em}}
\newcommand{\shrinkafter}{\vspace{-1.4em}}

\definecolor{verydarkgreen}{rgb}{0,0.2,0}
\definecolor{verydarkorange}{rgb}{0.4,0.2,0}
\definecolor{verydarkyellow}{rgb}{0.55,0.55,0}

%\newcommand{\changedshort}[1]{{\color{maroon}{#1}\normalfont}}
%\newcommand{\changed}[1]{{\color{dblue}{#1}\normalfont}}
%\newcommand{\changedb}[1]{{\color{verydarkgreen}{#1}\normalfont}}
%\newcommand{\changedc}[1]{{\color{verydarkorange}{#1}\normalfont}}
%\newcommand{\changedd}[1]{{\color{verydarkyellow}{#1}\normalfont}}
\newcommand{\changedshort}[1]{{#1}}
\newcommand{\changed}[1]{{#1}}
\newcommand{\changedb}[1]{{#1}}
\newcommand{\changedc}[1]{{#1}}
\newcommand{\changedd}[1]{{#1}}

\ifdefined\ShowNotes
\newcommand{\Connelly}[1]{\colornote{darkgreen}{CB:}{#1}}
\newcommand{\Adam}[1]{\colornote{dblue}{AF}{#1}}
\newcommand{\Yuting}[1]{\colornote{maroon}{YY}{#1}}
\newcommand{\todo}[1]{\colornote{darkgreen}{Todo}{#1}}
\newcommand{\changedf}[1]{{\color{dblue}{#1}\normalfont}}
\newcommand{\changedg}[1]{{\color{darkred}{#1}\normalfont}}
\newcommand{\changedh}[1]{{\color{verydarkgreen}{#1}\normalfont}}
\else
\newcommand{\Connelly}[1]{}
\newcommand{\Adam}[1]{}
\newcommand{\Yuting}[1]{}
\newcommand{\todo}[1]{}
\newcommand{\changedf}[1]{{#1}}
\newcommand{\changedg}[1]{{#1}}
\newcommand{\changedh}[1]{{#1}}
\fi

\ifdefined\ShowColor
\newcommand{\changedj}[1]{{\color{dblue}{#1}\normalfont}}
\newcommand{\changedi}[1]{{\changedj{#1}}}
\else
\newcommand{\changedj}[1]{{#1}}
\newcommand{\changedi}[1]{{#1}}
\fi

\newcommand{\tablegap}[0]{\\[-0.05cm]}
%\newcommand{\rottext}[2]{\raisebox{2.5\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{#1}}\hspace{0.03cm}\raisebox{2.5\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{#2}}}
\newcommand{\rottext}[2]{{\rotatebox[origin=c]{90}{#1}}\hspace{0.03cm}{\rotatebox[origin=c]{90}{#2}}}
\newcommand{\rottextfour}[4]{{\rotatebox[origin=c]{90}{#1}}\hspace{0.03cm}{\rotatebox[origin=c]{90}{#2}}\hspace{0.03cm}{\rotatebox[origin=c]{90}{#3}}\hspace{0.03cm}{\rotatebox[origin=c]{90}{#4}}}
%\newcommand{\change}[1]{{\color{verydarkgreen}{#1}\normalfont}}
%\newcommand{\changeb}[1]{{\color{verydarkblue}{#1}\normalfont}}
\newcommand{\change}[1]{{#1}}
\newcommand{\changeb}[1]{{#1}}

\newcommand{\videoframerate}[0]{1}

\newcommand{\treecannspeedup}[0]{12$\times$}
\newcommand{\kcoherencespeedup}[0]{9$\times$}
\newcommand{\patchmatchspeedup}[0]{200$\times$}

\ifdefined\ShowNotes
  \newcommand{\colornote}[3]{{\color{#1}\textbf{#2: #3}\normalfont}}
\else
  \newcommand{\colornote}[3]{}
\fi

\definecolor{darkred}{rgb}{0.7,0.1,0.1}
\definecolor{darkgreen}{rgb}{0.1,0.7,0.1}
\definecolor{verydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{verydarkblue}{rgb}{0.0,0.0,0.7}
\definecolor{cyan}{rgb}{0.7,0.0,0.7}
\definecolor{dblue}{rgb}{0.2,0.2,0.8}
\definecolor{maroon}{rgb}{0.76,.13,.28}
\definecolor{burntorange}{rgb}{0.81,.33,0}

\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}

\newcommand\fnurl[2]{%
  \href{#2}{#1}\footnote{\url{#2}}%
}

\definecolor{uhref_color}{HTML}{000066}

\newcommand\ulinec{\bgroup\markoverwith
      {\textcolor{uhref_color}{\rule[-0.5ex]{2pt}{0.4pt}}}\ULon}

\newcommand{\nsfurl}[1]{\ulinec{\small{\color{uhref_color}{\url{#1}}}}}


\newcommand{\beginintegraltable}[2]{
\begin{tabular}{|l|l|}
	\hline
	Function $f(x)$ &
	Bandlimited with #1 kernel: $\hat{f}^{(#2)}(x)$ \\
	\hline
}
\newcommand{\finishintegraltable}{
	\hline
	\end{tabular}\\ \\
}

\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\fract}{fract}
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\acos}{acos}
\DeclareMathOperator{\asin}{asin}
\DeclareMathOperator{\atan}{atan}

\newcommand\missing{} %\multicolumn{1}{|c|}{---}

%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}

\newcommand\tbltab{\hspace{0.25cm}}

\newcommand{\E}{\mathrm{E}}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{2\arrayrulewidth}


%%%%% Latin and language:
%% \newcommand{\etal       }     {\textit{et~al.}} old; not like ACM style
\newcommand{\etal       }     {{et~al.}}
\newcommand{\apriori    }     {\textit{a~priori}}
\newcommand{\aposteriori}     {\textit{a~posteriori}}
\newcommand{\perse      }     {\textit{per~se}}
\newcommand{\cf         }     {\textit{cf.}}
\newcommand{\eg         }     {{e.g.}}
\newcommand{\Eg         }     {{E.g.}}
\newcommand{\ie         }     {{i.e.}}
\newcommand{\Ie         }     {{I.e.}}
\newcommand{\vs         }     {{vs.}}
\newcommand{\naive      }     {{na\"{\i}ve}}

\newcommand{\half       }     {\ensuremath{\frac{1}{2}}}

% Paper-wide variables
\newcommand{\trace   }{\ensuremath{\mathcal{T}}}
\newcommand{\tracelen}{\ensuremath{\mathcal{N}}}
\newcommand{\reducedim}{\ensuremath{\mathcal{K}}}

% Shader names
\newcommand{\shadername}[1]{{\small\texttt{#1}}}
\newcommand{\bricks}{\shadername{Bricks}}
\newcommand{\marble}{\shadername{Marble}}
\newcommand{\mandelbulb}{\shadername{Mandel-bulb}}
\newcommand{\mandelbrot}{\shadername{Mandelbrot}}
\newcommand{\oceanic}{\shadername{Oceanic}}
\newcommand{\primitives}{\shadername{Gear}}
\newcommand{\gear}{\shadername{Gear}}
\newcommand{\trippy}{\shadername{Trippy}\,\shadername{Heart}}
\newcommand{\texturemap}{\shadername{Texture}\,\shadername{Maps}}
\newcommand{\venice}{\shadername{Venice}}

\newcommand{\shadertoy}{\href{https://www.shadertoy.com/}{\small\texttt www.shadertoy.com}}
\newcommand{\shadertoyshort}{\href{https://www.shadertoy.com/}{\small\texttt shadertoy}}

\newcommand{\rectdim}[2]{{{#1}$\times${#2}}}
\newcommand{\squaredim}[1]{{\rectdim{#1}{#1}}}

\newcommand{\spp}{{\textsc{spp}}}
\newcommand{\nspp}[1]{{{#1}\,\spp}}


==> Learning from Shader Program Traces (EG format)/9-notes.tex <==
\clearpage

\Yuting{Notes only, it's not part of the appendix.}

\section{P value on trace contubution hypothesis}

Null hypothesis:

\begin{equation}
    Pr[err_{good} \leq err_{subsample}] = \frac{1}{2}
\end{equation}

\begin{equation}
    Pr[err_{subsample} \leq err_{bad}] = \frac{1}{2}
\end{equation}

\subsection{Treat good < subsample < bad as one event}

\begin{equation}
    \begin{split}
        & Pr[err_{good} < err_{subsample} < err_{bad}] \\
        = & Pr[err_{good} \leq err_{subsample}] \cdot Pr[err_{subsample} \leq err_{bad}] \\
        = & \frac{1}{4}
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        & Pr[\text{other ordering}] \\
        = & 1 - Pr[err_{good} < err_{subsample} < err_{bad}] \\
        = & \frac{3}{4}
    \end{split}
\end{equation}

\subsubsection{All data points}

\begin{equation}
    \begin{split}
        & Pr[\text{other ordering happens at most 5 times out of 20}] \\
        = & \binom{20}{5} \cdot (\frac{3}{4})^5 \cdot (\frac{1}{4})^{15} \\
        + & \binom{20}{4} \cdot (\frac{3}{4})^4 \cdot (\frac{1}{4})^{16} \\
        + & \binom{20}{3} \cdot (\frac{3}{4})^3 \cdot (\frac{1}{4})^{17} \\
        + & \binom{20}{2} \cdot (\frac{3}{4})^2 \cdot (\frac{1}{4})^{18} \\
        + & \binom{20}{1} \cdot (\frac{3}{4})^1 \cdot (\frac{1}{4})^{19} \\
        + & \binom{20}{0} \cdot (\frac{1}{4})^{20} \\
        = & 3.8e-6
    \end{split}
\end{equation}

\subsubsection{Only one quater and one eighth}

\begin{equation}
    \begin{split}
        & Pr[\text{other ordering happens at most 0 times out of 8}] \\
        = & \binom{8}{0} \cdot (\frac{1}{4}) ^ 8 \\
        = & 1.5e-5
    \end{split}
\end{equation}

\subsubsection{Add bricks data at one quater}

\begin{equation}
    \begin{split}
        & Pr[\text{other ordering happens at most 1 times out of 9}] \\
        = & \binom{9}{1} \cdot (\frac{1}{4}) ^ 8 \cdot (\frac{3}{4})^1 \\
        + & \binom{9}{0} \cdot (\frac{1}{4}) ^ 9 \\
        = & 1.1e-4
    \end{split}
\end{equation}

\subsection{Treat good < subsample and subsample < bad independently}

\subsubsection{All data points}

\begin{equation}
    \begin{split}
        & Pr[(good > subsample) \text{ happens at most 3 times out of 20}] \\
        = & \binom{20}{3} \cdot (\frac{1}{2}) ^ 3 \cdot (\frac{1}{2})^{17} \\
        + & \binom{20}{2} \cdot (\frac{1}{2}) ^ 2 \cdot (\frac{1}{2})^{18} \\
        + & \binom{20}{1} \cdot (\frac{1}{2}) ^ 1 \cdot (\frac{1}{2})^{19} \\
        + & \binom{20}{0} \cdot (\frac{1}{2}) ^ 0 \cdot (\frac{1}{2})^{20} \\
        = & 0.00129
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        & Pr[(subsample > bad) \text{ happens at most 2 times out of 20}] \\
        = & \binom{20}{2} \cdot (\frac{1}{2}) ^ 2 \cdot (\frac{1}{2})^{18} \\
        + & \binom{20}{1} \cdot (\frac{1}{2}) ^ 1 \cdot (\frac{1}{2})^{19} \\
        + & \binom{20}{0} \cdot (\frac{1}{2}) ^ 0 \cdot (\frac{1}{2})^{20} \\
        = & 0.0002
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        Pr[\text{both event happens}] = 2.6e-7
    \end{split}
\end{equation}

\subsubsection{Only one quater and one eighth}

\begin{equation}
    \begin{split}
        & Pr[(good > subsample) \text{ happens at most 0 times out of 8}] \\
        = & \binom{8}{0} \cdot (\frac{1}{2})^8 \\
        = & 0.00390625
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        & Pr[(subsample > bad) \text{ happens at most 0 times out of 8}] \\
        = & \binom{8}{0} \cdot (\frac{1}{2})^8 \\
        = & 0.00390625
    \end{split}
\end{equation}

\begin{equation}
    Pr[\text{both event happens}] = 1.5e-5
\end{equation}

\subsubsection{Add bricks data at one quater}

\begin{equation}
    \begin{split}
        & Pr[(good > subsample) \text{ happens at most 1 times out of 9}] \\
        = & \binom{9}{1} \cdot (\frac{1}{2})^8 \cdot (\frac{1}{2})^9 \\
        + & \binom{9}{0} \cdot (\frac{1}{2})^9 \\
        = & 0.017578125
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        & Pr[(subsample > bad) \text{ happens at most 0 times out of 9}] \\
        = & \binom{9}{0} \cdot (\frac{1}{2})^9 \\
        = & 0.001953125
    \end{split}
\end{equation}

\begin{equation}
    Pr[\text{both event happens}] = 3.4e-5
\end{equation}

\section{Unified network: trace contribution to a certain channel in encoder's output channel}

Derived from equaiton 8 in https://arxiv.org/pdf/1611.06440.pdf

Because encoder contains only 1x1 conv, each pixel independently contributes to the output channel in the corresponding pixel position. Therefore, we could regard each pixel as an independent example (unlike in computing trace contribution for the entire network, pixels in the same feature map jointly contribute to the loss value).

We could simply use the abs value of the output channel as cost, because the taylor exapnsion will approximate the change in cost in either direction.

According to equation 8, this should be

\begin{equation}
    \text{score} = \sum_{\text{all pixels}} |\frac{\partial \mathbbm{O}}{\partial \mathbbm{I}} \mathbbm{I}|
\end{equation}

Here, both $\mathbbm{O}$ and $\mathbbm{I}$ are feature maps.

Tensorflow only allows computing the gradient of a scalar, so we have to make the following derivations.

Assume $m$ and $n$ are two distinct pixel indices in the feature map $m \neq n$. And since encoder contains only 1x1 conv, we have the following

\begin{equation}
    \frac{\partial \mathbbm{O}_m}{\partial \mathbbm{I}_n} = 0
\end{equation}

Therefore we could derive the gradient using the following scalar value

\begin{equation}
    \frac{\partial \sum_{\text{all pixels}} \mathbbm{O}_p}{\partial \mathbbm{I}_n} =  \sum_{\text{all pixels}} \frac{\partial \mathbbm{O}_p}{\partial \mathbbm{I}_n} = \frac{\partial\mathbbm{O}_n}{\partial \mathbbm{I}_n}
\end{equation}

The score for each trace can be rewritten into

\begin{equation}
    \begin{split}
        \text{score} = & \sum_{\text{all pixels}} |\frac{\partial \mathbbm{O}}{\partial \mathbbm{I}} \mathbbm{I}| \\
        = & \sum_{\text{all pixels}} |\frac{\partial \sum_{\text{all pixels}} \mathbbm{O}_p}{\partial \mathbbm{I}} \mathbbm{I}|
    \end{split}
\end{equation}

\section{Current Result}

\input{figtex/result_pool}

\ignorethis{

\Yuting{These are notes from last subsmission.}

\input{figtex/supp_denoising_table.tex}

Things we need to work on in the paper:
\begin{itemize}
\item 
Changes to how we handle branching, loops
- Clustering, every nth --- this is done in ablation experiment for Mandelbrot, should double check that we talk about it.

\item
Tiled training 
- integrate tiled rendering

\item
Postprocessing filters

\item
Y can update figures for post processing

\item
Ablation study: All, no perceptual, no L2, fewer layers, first 5, last 5, .... \Connelly{figures are updated, need to check that text is updated.}

\item
Update abstract to reflect postprocessing effects and other changes

\end{itemize}

Finished items (leaving the list so we can double check later in an editing pass):

\begin{itemize}
\item
Perceptual error --- changed loss in Sect 4.4

\item
Sigma on input

\item
Put in figure captions perceptual, L2 and perceptual --- \Connelly{Y and I think we decided not to do this}

\item
Texture experiments: one takes both branches, one zeroes out the path not taken
- branch not taken experiment

\item
Analyze features that are important \Connelly{Yuting is working on this}



%\input{figtex/result_pool.tex}

\end{itemize}

}

==> Learning from Shader Program Traces (EG format)/a0-description.tex <==
\begin{center}
{\LARGE Appendices} \\ \vspace{0.5\baselineskip}
{\Large \textit{Learning from Shader Program Traces}} \\ \vspace{0.5\baselineskip}
(in review for Eurographics 2022)
\end{center}

\emph{Note to reviewers:} Here we include as appendices some details we removed from the main body of the paper to reduce overall length. Any or all them could be included or omitted as needed.

==> Learning from Shader Program Traces (EG format)/figtex/arch.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=3.25in]{figures/architecture_v6.pdf}
    \caption{Network architecture used in our experiments. The input from the program trace has \tracelen\ channels. The output layer has three channels for color images. \changedi{The first feature reduction layer has \reducedim\ channels. We use $\reducedim = 48$ in our method. When training the baseline method, \reducedim\ will be increased to a larger value to match the total number of trainable weights to be the same as training with the program trace at the maximum length.} All \changedi{other} intermediate layers have 48 channels. The input feature maps are first analyzed by four 1x1 convolutional layers, followed by five 3x3 convolutional layers with dilation rates of ${1, 2, 4, 8, 1}$ respectively. Finally, four additional 1x1 convolutional layers are applied and output a three channel image. Note that the first and last convolutional blocks indicated in lighter blue each reduce the number of channels (from \tracelen\ to 48, and from 48 to 3, respectively).}
    \label{fig:architecture}
\end{figure}


==> Learning from Shader Program Traces (EG format)/figtex/error-table-data.tex <==
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Shader}} & \multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{2}{c}{Perceptual (\%)} & \multicolumn{2}{c}{L2 Error (\%)} \\ \cline{3-6}
\multicolumn{1}{c|}{} & Distances: & Similar & Different & Similar & Different  \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\oceanic \\ Fig. 1 \\ \tracelen\ = 702\end{tabular}}} & Ours & \textbf{2.85} & \textbf{3.19} & \textbf{1.83} & \textbf{1.86} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 3.34 & 3.72 & 2.04 & 2.05 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 41.62 & 45.23 & 6.46 & 6.75 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\bricks \\ Fig. 2 \\ \tracelen\ = 56\end{tabular}}} & Ours & \textbf{0.23} & \textbf{0.66} & \textbf{0.61} & \textbf{0.83} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 0.66 & 2.43 & 0.97 & 1.45 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 19.12 & 24.34 & 4.75 & 6.55 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb \\ Fig. 2 \\ \tracelen\ = 232\end{tabular}}} & Ours & \textbf{0.51} & \textbf{0.62} & \textbf{1.41} & \textbf{1.40} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 0.81 & 0.93 & 1.76 & 1.65 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 4.84 & 5.92 & 3.04 & 3.15 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\marble \\ Fig. 2 \\ \tracelen\ = 226\end{tabular}}} & Ours & \textbf{1.96} & \textbf{2.68} & \textbf{2.75} & \textbf{2.97} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 3.28 & 5.22 & 3.69 & 3.93 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 23.92 & 28.96 & 13.34 & 15.59 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\texturemap \\ Fig. 2 \\ \tracelen\ = 80\end{tabular}}} & Ours & \textbf{2.15} & \textbf{6.19} & \textbf{1.66} & \textbf{2.31} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 2.86 & 6.77 & 1.88 & 2.42 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 29.77 & 34.77 & 6.12 & 7.81 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\primitives \\ Fig. 5 \\ \tracelen\ = 771\end{tabular}}} & Ours & \textbf{0.96} & \textbf{0.94} & \textbf{1.05} & \textbf{1.06} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 1.23 & 1.17 & 1.10 & 1.11 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 15.37 & 16.24 & 3.26 & 3.28 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\trippy \\ Fig. 5 \\ \tracelen\ = 199\end{tabular}}} & Ours & \textbf{5.37} & \textbf{5.54} & \textbf{4.35} & \textbf{4.44} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 7.17 & 6.50 & 4.91 & 4.84 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 23.13 & 19.91 & 7.84 & 7.54 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot \\ Fig. 5 \\ \tracelen\ = 131\end{tabular}}} & Ours & \textbf{0.31} & \textbf{0.35} & \textbf{1.17} & \textbf{1.15} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 0.83 & 1.07 & 1.55 & 1.51 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 23.40 & 19.95 & 6.79 & 6.22 \\ \hline

\end{tabular}

==> Learning from Shader Program Traces (EG format)/figtex/error-table-new.tex <==
\begin{table}
\centering
\caption{Error statistics for shaders in Figures \ref{fig:teaser}, \ref{fig:result_fig1} and \ref{fig:result_fig2}. We report errors for test datasets with similar and different distances to the geometry: see \sect{sec:dataset} for  details. Note that elsewhere in the paper, we simply report a single mean error over the test set. For each test dataset, we report metrics for mean RGB $L^2$ error and perceptual error \cite{zhang2018perceptual}.}
\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}

\input{figtex/error-table-data}

\label{tab:error_breakdown}
\vspace{-2ex}
\end{table}

==> Learning from Shader Program Traces (EG format)/figtex/error_table_denoising.tex <==
\setlength{\tabcolsep}{10pt}
\begin{table*}[]
\centering
\caption{Error statistics for denoising (\sect{sec:denoising}). We report LPIPS perceptual error \cite{zhang2018perceptual}, SSIM and PSNR. The numbers reported are averaged across the entire test dataset. 
%
The error metric in the first two columns (RGBx and ours) are already reported in the main paper \tbl{tab:err_main}, we include them here for a clear comparison with Supersampling.
%
For LPIPS, we report the absolute error for the RGBx baseline, and for other methods their errors relative to that of the RGBx baseline (\% or $\times$).}

\begin{tabular}{l|c@{ / }c@{ / }cc@{ / }c@{ / }cc@{(}r@{) / }c@{ / }c}
    \hline
    
    Shader & \multicolumn{3}{c}{RGBx} & \multicolumn{3}{c}{Ours} & \multicolumn{4}{c}{Supersampling} \\ \hline
    
            \bricks & 0.0141 & 0.981 & 36.68 & \textbf{0.0097(68\%)} & \textbf{0.987} & \textbf{38.29} & 0.2985 & 21$\times$ & 0.839 & 24.14 \\ \hline
            \gear & 0.0173 & 0.986 & 38.90 & \textbf{0.0127(73\%)} & \textbf{0.988} & \textbf{39.86} & 0.2935 & 17$\times$ & 0.880 & 24.71 \\ \hline
            \mandelbrot & 0.0235 & 0.973 & 36.07 & \textbf{0.0059(24\%)} & \textbf{0.986} & \textbf{38.55} & 0.3502 & 15$\times$ & 0.746 & 23.46 \\ \hline
            \mandelbulb & 0.0185 & 0.962 & 32.14 & \textbf{0.0118(63\%)} & \textbf{0.975} & \textbf{34.18} & 0.1580 & 8.5$\times$ & 0.895 & 23.98 \\ \hline
            \oceanic & 0.0403 & 0.961 & 33.69 & \textbf{0.0339(84\%)} & \textbf{0.966} & \textbf{34.51} & 0.4314 & 11$\times$ & 0.780 & 23.81 \\ \hline
            \trippy & 0.0696 & 0.856 & 26.30 & \textbf{0.0543(77\%)} & \textbf{0.886} & \textbf{27.27} & 0.2178 & 3.1$\times$ & 0.767 & 22.42 \\ \hline
            \venice & 0.0309 & 0.965 & 32.76 & \textbf{0.0242(78\%)} & \textbf{0.973} & \textbf{33.83} & 0.2893 & 9.4$\times$ & 0.853 & 23.73 \\ \hline
    
    
    
\end{tabular}
%\vspace{-1ex}

\label{tab:error_denoising}
\end{table*}

==> Learning from Shader Program Traces (EG format)/figtex/error_table_main.tex <==

\setlength{\tabcolsep}{2.5pt}
\begin{table}[t]

\centering

\caption{Error statistics for applications in \sect{sec:eval} and \ref{sec:multiple_shaders}. Errors reported as LPIPS \cite{zhang2018perceptual} / SSIM / PSNR. 
%For LPIPS we report both absolute error and our relative error (\%) compared to RGBx, as in \fig{fig:summary_bar}.
}

\begin{tabular}{c|l|c@{ / }c@{ / }cc@{ / }c@{ / }c}
        \hline
         & Shader & \multicolumn{3}{c}{RGBx} & \multicolumn{3}{c}{Ours} \\ \thickhline
        
        {\multirow{7}{*}{\rotatebox[origin=c]{90}{Denoising}}} & \bricks & 0.0141 & 0.981 & 36.68 & \textbf{0.0097} & \textbf{0.987} & \textbf{38.29} \\ 
     \cline{2-8} 
                         & \gear & 0.0173 & 0.986 & 38.90 & \textbf{0.0127} & \textbf{0.988} & \textbf{39.86} \\ 
     \cline{2-8} 
                         & \mandelbrot & 0.0235 & 0.973 & 36.07 & \textbf{0.0059} & \textbf{0.986} & \textbf{38.55} \\ 
     \cline{2-8} 
                         & \mandelbulb & 0.0185 & 0.962 & 32.14 & \textbf{0.0118} & \textbf{0.975} & \textbf{34.18} \\ 
     \cline{2-8} 
                         & \oceanic & 0.0403 & 0.961 & 33.69 & \textbf{0.0339} & \textbf{0.966} & \textbf{34.51} \\ 
     \cline{2-8} 
                         & \trippy & 0.0696 & 0.856 & 26.30 & \textbf{0.0543} & \textbf{0.886} & \textbf{27.27} \\ 
     \cline{2-8} 
                         & \venice & 0.0309 & 0.965 & 32.76 & \textbf{0.0242} & \textbf{0.973} & \textbf{33.83} \\ 
     \thickhline 
        {\multirow{5}{*}{\rotatebox[origin=c]{90}{Simplified}}} & \bricks & 0.0624 & 0.922 & 25.57 & \textbf{0.0398} & \textbf{0.936} & \textbf{29.96} \\ 
     \cline{2-8} 
                         & \mandelbrot & 0.1111 & 0.826 & 27.04 & \textbf{0.0430} & \textbf{0.949} & \textbf{31.15} \\ 
     \cline{2-8} 
                         & \mandelbulb & 0.0932 & 0.812 & 25.22 & \textbf{0.0600} & \textbf{0.856} & \textbf{26.85} \\ 
     \cline{2-8} 
                         & \trippy & 0.2412 & 0.520 & 18.55 & \textbf{0.1824} & \textbf{0.629} & \textbf{20.95} \\ 
     \cline{2-8} 
                         & \venice & 0.0404 & 0.957 & 31.50 & \textbf{0.0285} & \textbf{0.965} & \textbf{32.72} \\ 
     \thickhline 
        {\multirow{3}{*}{\rotatebox[origin=c]{90}{Post}}} & blur & 0.0126 & 0.978 & 35.81 & \textbf{0.0082} & \textbf{0.985} & \textbf{37.62} \\ 
     \cline{2-8} 
                         & Sharpen & 0.0881 & 0.833 & 24.26 & \textbf{0.0693} & \textbf{0.868} & \textbf{25.31} \\ 
     \cline{2-8} 
                         & Simp Sharpen & 0.2675 & 0.477 & 17.20 & \textbf{0.2154} & \textbf{0.587} & \textbf{19.35} \\ 
     \thickhline 
     {\multirow{4}{*}{\rotatebox[origin=c]{90}{Shared}}} & \gear & 0.0251 & 0.984 & 38.16 & \textbf{0.0173} & \textbf{0.986} & \textbf{38.66} \\ 
     \cline{2-8} 
                         & \mandelbrot & 0.0546 & 0.801 & 28.02 & \textbf{0.0165} & \textbf{0.933} & \textbf{32.60} \\ 
     \cline{2-8} 
                         & \mandelbulb & 0.0423 & 0.861 & 28.02 & \textbf{0.0298} & \textbf{0.906} & \textbf{30.19} \\ 
     \cline{2-8} 
                         & \trippy & 0.1048 & 0.815 & 19.99 & \textbf{0.0755} & \textbf{0.857} & \textbf{23.88} \\ 
     \thickhline 
    \end{tabular}

\label{tab:err_main}

\vspace{-2ex}
\end{table}

==> Learning from Shader Program Traces (EG format)/figtex/error_table_post_processing.tex <==
\setlength{\tabcolsep}{4.0pt}
\begin{table}[]
\caption{Errors learning postprocessing filters, as in \tbl{tab:error_denoising}. \changedi{Each postprocessing filter is trained with a specific shader: blur (\mandelbulb), sharpen (\trippy) and simplified sharpen (\trippy).}}
\vspace{-0.75\baselineskip}
\begin{tabular}{l|r@{}l@{ / }r@{}lr@{\%}l@{ / }r@{\%}l}
    \hline

        Shader & \multicolumn{4}{c}{RGBx} & \multicolumn{4}{c}{Ours} \\ \thickhline
    
         blur & 1.2 & e-02 & 3.6 & e-04 & \textbf{65} & & \textbf{69} & \\ \hline
         sharpen & 8.8 & e-02 & 3.8 & e-03 & \textbf{78} & & \textbf{78} & \\ \hline
         simp sharpen & 2.7 & e-01 & 2.0 & e-02 & \textbf{80} & & \textbf{60} & \\ \hline
    \end{tabular}
\label{tab:error_post_processing}
\end{table}

==> Learning from Shader Program Traces (EG format)/figtex/error_table_simplified.tex <==
\vspace{-1ex}
\setlength{\tabcolsep}{4.0pt}
\begin{table}[]
\caption{Errors reconstructing simplified shaders, as in \tbl{tab:error_denoising}.}
\vspace{-0.75\baselineskip}
\begin{tabular}{l|r@{}l@{ / }r@{}lr@{\%}l@{ / }r@{\%}l}
    \hline

        Shader & \multicolumn{4}{c}{RGBx} & \multicolumn{4}{c}{Ours} \\ \thickhline
    
         \bricks & 6.3 & e-02 & 3.0 & e-03 & \textbf{63} & & \textbf{46} & \\ \hline
         \mandelbrot & 1.1 & e-01 & 3.7 & e-03 & \textbf{38} & & \textbf{45} & \\ \hline
         \mandelbulb & 9.3 & e-02 & 5.4 & e-03 & \textbf{64} & & \textbf{72} & \\ \hline
         \trippy & 2.4 & e-01 & 1.5 & e-02 & \textbf{75} & & \textbf{57} & \\ \hline
         \venice & 4.0 & e-02 & 7.2 & e-04 & \textbf{70} & & \textbf{74} & \\ \hline
    \end{tabular}
\label{tab:error_simplified}
\end{table}

==> Learning from Shader Program Traces (EG format)/figtex/error_table_temporal.tex <==

\setlength{\tabcolsep}{2pt}
\begin{table}[!bt]

\centering

\caption{Error statistic for learning temporally coherence sequences.
%
Metrics reported are similar as in \tbl{tab:err_main}.
%
The temporal application is trained both on shaders with full computation and simplified shaders with partial computation (simp). For each experiment, we generate a 30 frames sequence and compute the error with respect to ground truth using the last frame. The reported numbers are averaged across 30 different sequences.
}

\begin{tabular}{l|c@{ / }c@{ / }cc@{ / }c@{ / }c}
        \hline
        Shader & \multicolumn{3}{c}{RGBx} & \multicolumn{3}{c}{Ours} \\ \thickhline
        
        \mandelbrot\  & 0.0104 & 0.980 & 37.16 & \textbf{0.0037} & \textbf{0.989} & \textbf{39.75} \\ 
     \cline{1-7} 
                         \mandelbrot\ simp  & 0.1049 & 0.898 & 27.51 & \textbf{0.0693} & \textbf{0.929} & \textbf{28.93} \\ 
     \cline{1-7}
                         \mandelbulb\  & 0.0213 & 0.959 & 32.06 & \textbf{0.0140} & \textbf{0.971} & \textbf{33.56} \\ 
     \cline{1-7}
                         \mandelbulb\ simp  & 0.1194 & 0.780 & 23.49 & \textbf{0.1035} & \textbf{0.788} & \textbf{24.25} \\ 
     \cline{1-7}
                         \trippy\  & 0.0665 & 0.864 & 26.61 & \textbf{0.0546} & \textbf{0.884} & \textbf{27.17} \\ 
     \cline{1-7}
                         \trippy\ simp  & 0.2295 & 0.563 & 19.10 & \textbf{0.1788} & \textbf{0.637} & \textbf{21.10} \\ 
     \thickhline 
    \end{tabular}

\vspace{2ex}

\label{tab:err_temporal}
\end{table}

==> Learning from Shader Program Traces (EG format)/figtex/error_table_unified.tex <==
\vspace{-1ex}
\setlength{\tabcolsep}{4.0pt}
\begin{table}[]
\caption{\changedi{Errors training a shared denoiser for \mandelbrot, \mandelbulb, \primitives\ and \trippy, as in \tbl{tab:error_denoising}.}}
\vspace{-0.75\baselineskip}
\begin{tabular}{l|r@{}l@{ / }r@{}lr@{\%}l@{ / }r@{\%}l}
    \hline

        Shader & \multicolumn{4}{c}{RGBx} & \multicolumn{4}{c}{Ours} \\ \thickhline
    
         \mandelbrot & 5.4 & e-02 & 1.9 & e-03 & \textbf{30} & & \textbf{35} & \\ \hline
         \mandelbulb & 4.3 & e-02 & 2.0 & e-03 & \textbf{70} & & \textbf{59} & \\ \hline
         \primitives & 2.5 & e-02 & 1.7 & e-04 & \textbf{69} & & \textbf{85} & \\ \hline
         \trippy & 1.0 & e-01 & 1.1 & e-02 & \textbf{72} & & \textbf{40} & \\ \hline
\end{tabular}
\label{tab:error_unified}
\end{table}

==> Learning from Shader Program Traces (EG format)/figtex/mandelbrot_ablation.tex <==
\begin{figure*}
  \setlength{\tabcolsep}{1pt}
  \setlength{\h}{1.14in}
  \vspace{3\baselineskip}
  \begin{tabular}{cccccccc}
  
(a) L2 & (b) Perceptual & (c) All & (d) Every 4th & (e) First 5 & (f) Last 5 & (g) Subsample 4 & (h) Mean \& Var \\
\addlinespace[4pt]
  
 \includegraphics[height=\h]{results/mandelbrot_l2_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_perceptual_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_all_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_every_4th_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_first_5_no_last_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_last_5_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_subsample_4_zoom_thin.png} &  \includegraphics[height=\h]{results/mandelbrot_mean_var_zoom_thin.png} \tablegap

 
{\small 189 ms, 0.65\%} & 
{\small 201 ms, 0.33\%} & 
{\small 265 ms, 0.29\%} &
{\small 226 ms, 0.33\%} & 
{\small 193 ms, 0.35\%} & 
{\small 196 ms, 0.40\%} &
{\small 200 ms, 0.39\%} &
{\small 212 ms, 0.38\%} \\
  
  \end{tabular}
  \vspace{-2ex}
  \caption{Ablation study for shader \mandelbrot. We show our method, with the same zoom regions as in \fig{fig:result_fig2}. Time and error values are reported below each image as in Figure 1. We train a total of 400 epochs for each experiment. In (a-b) we report ablations on the training loss selection, where \mandelbrot's loop is handled the same as in \fig{fig:result_fig2}. (a) L2 loss only; (b) Perceptual loss only. The errors in (a-b) are higher, and thin line structures are broken or blurred. Thus, our method of combining both L2 and perceptual loss is the best. In (c-h) we show the different options for handling loops mentioned in \sect{sec:loops}: we handle the loop by unrolling (c) or sample every 4th trace from the entire program (d), or add to the trace only the first (e) or last (f) 5 iterations of the loop, subsample every 4 iterations (g) or collect mean and variance statistics from all loop iterations (h). (c) is slower than (d-h) because a longer trace must be gathered. (d-h) are slightly visually and quantitatively worse than using all loop iterations (c), but much faster. For comparison, the \mandelbrot\ shader that we selected in \fig{fig:result_fig2} uses the first 5 and last 1 loop iterations: this gives a slightly better visual and quantitative result in a similar running time.}
  \label{fig:mandelbrot_ablation}
\end{figure*}

==> Learning from Shader Program Traces (EG format)/figtex/postprocessing.tex <==
\begin{figure}
\centering
\setlength{\h}{1.5in}
    \centering
    \begin{tabular}{cc}
(a) Ground Truth & (b) Our result \\
\includegraphics[width=\h]{results/postprocessing_defocus_blur_gt.png} & \includegraphics[width=\h]{results/postprocessing_defocus_blur_ours.png} \\
\small{\mandelbulb: defocus} & \small{Perceptual: 0.4\%, L2: 1.2\%} \\ \\
\includegraphics[width=\h]{results/postprocessing_sharpen_gt.png} & \includegraphics[width=\h]{results/postprocessing_sharpen_ours.png} \\
\small{\trippy: sharpen} & \small{Perceptual: 6.9\%, L2: 5.5\%}
\end{tabular}
    \caption{Result images for postprocessing filters: defocus for \mandelbulb\ and sharpen for \trippy. Under our result we report both perceptual and L2 error over the test set.}
    \label{fig:postprocessing}
\end{figure}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig1.tex <==
\begin{figure*}
\ResultsFigWithHeader{\bricks}{bricks}{688 sec}{751 ms, 0.4}{754 ms, 1.3}{\nspp{1}, 688\,ms, 21}
\ResultsFigNoHeader{\mandelbulb}{mandelbulb}{47 sec}{143 ms, 0.5}{115 ms, 0.8}{\nspp{3}, 141\,ms, 5}
\ResultsFigNoHeader{\marble}{marble2}{714 sec}{785 ms, 2.2}{747 ms, 3.9}{\nspp{1}, 714\,ms, 26}
\ResultsFigNoHeader{\texturemap}{texture_map3}{1111 sec}{1177 ms, 3.5}{1165 ms sec, 4.2}{\nspp{1}, 1111\,ms, 31}
  \vspace{-2ex}
  \caption{Denoising shaders \bricks, \mandelbulb, \marble\ and \texturemap. Time and error values are as in Figure 1. Our method better recovers both the orientation and high-frequency detail than the baseline methods.} 
  \label{fig:result_fig1}
  \vspace{-1ex}
\end{figure*}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig2.tex <==
\begin{figure*}
\ResultsFigWithHeader{\primitives}{primitives}{1123 sec}{1325 ms, 1.0}{1217 ms, 1.2}{\nspp{1}, 1123\,ms, 16}
\ResultsFigNoHeader{\trippy}{trippy}{30 sec}{123 ms, 5.4}{97.6 ms, 6.9}{\nspp{4}, 121\,ms, 22}
\ResultsFigNoHeader{\mandelbrot}{mandelbrot}{106 sec}{202 ms, 0.32}{185 ms, 0.91}{\nspp{2}, 212\,ms, 22}
  \vspace{-2ex}
  \caption{Result images for shaders \primitives, \trippy, and \mandelbrot. Time and error values are reported below each image as in Figure 1. For \primitives, our method better recovers the orientation and high-frequency detail of the 3D geometry. For \trippy, our method better reproduces high-frequency texture. For \mandelbrot, our method better preserves thin line structures.}
  \label{fig:result_fig2}
\end{figure*}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig_def.tex <==
\newcommand{\ResultsFigStart}{
\setlength{\tabcolsep}{1pt}
\setlength{\h}{1.15in}
\begin{tabular}{cccccc}
}


\newcommand{\ResultsFigWithHeader}[6]{
\ResultsFigStart
(a) Reference & (b) Our result & (c) Reference & (d) Ours & (e) RGB+Aux & (f) Supersample\\
\addlinespace[4pt]
\ResultsFigEnd{#1}{#2}{#3}{#4}{#5}{#6}
}

\newcommand{\ResultsFigNoHeader}[6]{
\addlinespace[4pt]
\ResultsFigStart
\ResultsFigEnd{#1}{#2}{#3}{#4}{#5}{#6}
}

%%%%%%%%%%%%%%%%%%%%%%%
% Start of macros for new fig
% can delete the above macros once old figures are replaced
%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%
% macro for teaser (4 img + zoom)
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ResultsFigStartTeaser}{
\setlength{\tabcolsep}{1pt}
\setlength{\h}{1.03in}
\begin{tabular}{cc@{\hskip 4pt}cc@{\hskip 4pt}cc@{\hskip 4pt}cc}
}


\newcommand{\ResultsFigEndTeaser}[5]{
\includegraphics[height=\h]{result_figs/#2_gt_box.png} & \includegraphics[height=\h]{result_figs/#2_gt_zoom.png} & \includegraphics[height=\h]{result_figs/#2_input_box.png} & \includegraphics[height=\h]{result_figs/#2_input_zoom.png} & \includegraphics[height=\h]{result_figs/#2_RGBx_box.png} & \includegraphics[height=\h]{result_figs/#2_RGBx_zoom.png} & \includegraphics[height=\h]{result_figs/#2_ours_box.png} & \includegraphics[height=\h]{result_figs/#2_ours_zoom.png} \tablegap
\multicolumn{2}{c}{\small {#1}} &
\multicolumn{2}{c}{\small {#3}} &
\multicolumn{2}{c}{\small {#4}} &
\multicolumn{2}{c}{\small {#5}}
\end{tabular}
}

\newcommand{\ResultsFigTeaser}[5]{
\ResultsFigStartTeaser
\multicolumn{2}{c}{(a) Reference} & \multicolumn{2}{c}{(b) Simplified Input} & \multicolumn{2}{c}{(c) RGBx Baseline} & \multicolumn{2}{c}{(d) Our Result} \\
\addlinespace[4pt]
\ResultsFigEndTeaser{#1}{#2}{#3}{#4}{#5}
}

%%%%%%%%%%%%%%%%%%%%%%%
% macro for denoising (2 full img + 4 zooms)
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ResultsFigStartWithZoom}{
\setlength{\tabcolsep}{1pt}
\setlength{\h}{1.15in}
\begin{tabular}{cccccc}
}

\newcommand{\ResultsFigEndWithZoom}[6]{
\includegraphics[height=\h]{result_figs/#2_gt_box.png} & \includegraphics[height=\h]{result_figs/#2_ours_box.png} & \includegraphics[height=\h]{result_figs/#2_gt_zoom.png} & \includegraphics[height=\h]{result_figs/#2_MSAA_zoom.png} & \includegraphics[height=\h]{result_figs/#2_RGBx_zoom.png} & 
\includegraphics[height=\h]{result_figs/#2_ours_zoom.png} \tablegap
{\small {#1}} & & 
{\small {#3}} & 
{\small {#6}} & 
{\small {#5}} & 
{\small {#4}} 
\end{tabular}
}

\newcommand{\ResultsFigWithHeaderWithZoom}[6]{
\ResultsFigStartWithZoom
(a) Reference & (b) Our Result & (c) Reference & (d) Supersample & (e) RGBx & (f) Ours\\
\addlinespace[4pt]
\ResultsFigEndWithZoom{#1}{#2}{#3}{#4}{#5}{#6}
}

\newcommand{\ResultsFigNoHeaderWithZoom}[6]{
\ResultsFigStartWithZoom
\addlinespace[4pt]
\ResultsFigEndWithZoom{#1}{#2}{#3}{#4}{#5}{#6}
}

\newcommand{\ResultsFigEndWithCorrectedZoom}[6]{
\includegraphics[height=\h]{result_figs/#2_gt_box.png} & \includegraphics[height=\h]{result_figs/#2_ours_box.png} & \includegraphics[height=\h]{result_figs/#2_corrected_gt_zoom.png} & \includegraphics[height=\h]{result_figs/#2_corrected_MSAA_zoom.png} & \includegraphics[height=\h]{result_figs/#2_corrected_RGBx_zoom.png} & 
\includegraphics[height=\h]{result_figs/#2_corrected_ours_zoom.png} \tablegap
{\small {#1}} & & 
{\small {#3}} & 
{\small {#6}} & 
{\small {#5}} & 
{\small {#4}} 
\end{tabular}
}

\newcommand{\ResultsFigWithHeaderWithCorrectedZoom}[6]{
\ResultsFigStartWithZoom
(a) Reference & (b) Our Result & (c) Reference & (d) Supersample & (e) RGBx & (f) Ours\\
\addlinespace[4pt]
\ResultsFigEndWithCorrectedZoom{#1}{#2}{#3}{#4}{#5}{#6}
}

\newcommand{\ResultsFigNoHeaderWithCorrectedZoom}[6]{
\ResultsFigStartWithZoom
\addlinespace[4pt]
\ResultsFigEndWithCorrectedZoom{#1}{#2}{#3}{#4}{#5}{#6}
}

%%%%%%%%%%%%%%%%%%%%%%%
% macro for simplified (2 full img and 4 zooms)
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ResultsFigEndInputWithZoom}[6]{
\includegraphics[height=\h]{result_figs/#2_gt_box.png} & \includegraphics[height=\h]{result_figs/#2_ours_box.png} & \includegraphics[height=\h]{result_figs/#2_gt_zoom.png} & \includegraphics[height=\h]{result_figs/#2_input_zoom.png} & \includegraphics[height=\h]{result_figs/#2_RGBx_zoom.png} & 
\includegraphics[height=\h]{result_figs/#2_ours_zoom.png} \tablegap
{\small {#1}} & & 
{\small {#3}} & 
{\small {#6}} & 
{\small {#5}} & 
{\small {#4}} 
\end{tabular}
}

\newcommand{\ResultsFigWithHeaderInputWithZoom}[6]{
\ResultsFigStartWithZoom
(a) Reference & (b) Our Result & (c) Reference & (d) Input & (e) RGBx & (f) Ours\\
\addlinespace[4pt]
\ResultsFigEndInputWithZoom{#1}{#2}{#3}{#4}{#5}{#6}
}

\newcommand{\ResultsFigNoHeaderInputWithZoom}[6]{
\ResultsFigStartWithZoom
\addlinespace[4pt]
\ResultsFigEndInputWithZoom{#1}{#2}{#3}{#4}{#5}{#6}
}

%%%%%%%%%%%%%%%%%%%%%%%
% macro for simplified (4 full img)
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ResultsFigStartWithoutZoom}{
\setlength{\tabcolsep}{1pt}
\setlength{\h}{1.15in}
\begin{tabular}{cccc}
}

\newcommand{\ResultsFigEndWithoutZoom}[5]{
\includegraphics[height=\h]{result_figs/#2_gt.png} & \includegraphics[height=\h]{result_figs/#2_input.png} & \includegraphics[height=\h]{result_figs/#2_RGBx.png} & \includegraphics[height=\h]{result_figs/#2_ours.png} \tablegap
{\small {#1}} & {\small {#5}} &
{\small {#4}} & 
{\small {#3}} 
\end{tabular}
}

\newcommand{\ResultsFigWithHeaderWithoutZoom}[5]{
\ResultsFigStartWithoutZoom
(a) Reference & (b) Simplified Input & (c) RGBx Baseline & (d) Our Result \\
\addlinespace[4pt]
\ResultsFigEndWithoutZoom{#1}{#2}{#3}{#4}{#5}
}

\newcommand{\ResultsFigNoHeaderWithoutZoom}[5]{
\ResultsFigStartWithoutZoom
\addlinespace[4pt]
\ResultsFigEndWithoutZoom{#1}{#2}{#3}{#4}{#5}
}

%%%%%%%%%%%%%%%%%%%%%%%
% macro for post processing (3 cropped img + zoom)
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ResultsFigStartThreeCol}{
\setlength{\tabcolsep}{1pt}
\setlength{\h}{1.15in}
\begin{tabular}{cc@{\hskip 4pt}cc@{\hskip 4pt}cc}
}

\newcommand{\ResultsFigEndThreeCol}[4]{
\includegraphics[height=\h]{result_figs/#2_gt_box.png} & \includegraphics[height=\h]{result_figs/#2_gt_zoom.png} & \includegraphics[height=\h]{result_figs/#2_RGBx_box.png} & \includegraphics[height=\h]{result_figs/#2_RGBx_zoom.png} & \includegraphics[height=\h]{result_figs/#2_ours_box.png} & \includegraphics[height=\h]{result_figs/#2_ours_zoom.png} \tablegap
\multicolumn{2}{c}{\small {#1}} &
\multicolumn{2}{c}{\small {#3}} &
\multicolumn{2}{c}{\small {#4}} 
\end{tabular}
}

\newcommand{\ResultsFigWithHeaderThreeCol}[4]{
\ResultsFigStartThreeCol
\multicolumn{2}{c}{(a) Reference} & \multicolumn{2}{c}{(b) RGBx Baseline} & \multicolumn{2}{c}{(c) Our Result} \\
\addlinespace[4pt]
\ResultsFigEndThreeCol{#1}{#2}{#3}{#4}
}

\newcommand{\ResultsFigNoHeaderThreeCol}[4]{
\ResultsFigStartThreeCol
\addlinespace[4pt]
\ResultsFigEndThreeCol{#1}{#2}{#3}{#4}
}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig_denoising.tex <==
\begin{figure*}

\ResultsFigWithHeaderWithZoom{\bricks}{new_submission/denoising_bricks}{0\%/1x}{68\%/930x}{100\%/960x}{1\,SPP, 21x/1000x}

\ResultsFigNoHeaderWithZoom{\mandelbrot}{new_submission/denoising_mandelbrot}{0\%/1x}{24\%/740x}{100\%/780x}{2\,SPP, 15x/520x}

\ResultsFigNoHeaderWithZoom{\oceanic}{new_submission/denoising_oceanic}{0\%/1x}{83\%/990x}{100\%/1000x}{1\,SPP, 11x/1000x}
    
\ResultsFigNoHeaderWithZoom{\primitives}{new_submission/denoising_primitives2}{0\%/1x}{74\%/960x}{100\%/980x}{1\,SPP, 17x/1000x}

\vspace{-2ex}
\caption{Learning to reduce sampling noise in procedural shaders.
%
The reference low-noise solution (a) relies on 1000 samples per pixel (\spp). Our method (b) approximates the reference well at only \nspp{1}. Zooming into the region boxed in green (c, f) reveals approximation error, which compares favorably with the two baselines: (d) supersampling where the number of samples is chosen to have comparable run-time as ours, and (e) RGBx.
%
Error and speedups are reported as in \fig{fig:teaser}.
%We report relative perceptual error over a test set compared with the RGBx baseline (e) and relative speedup compared with reference solution (c) in the format of error/speedup. 
%
Our method better covers both the orientation and high-frequency detail than the baselines. 
%
\bricks\ and \mandelbrot\ are gamma corrected to emphasize visual differences.
%when viewed on screens of various brightness. 
%Full images for all experiments can be found in the supplemental material.
}
\vspace{-4ex}
\label{fig:result_denoising}
\end{figure*}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig_denoising1.tex <==
\begin{figure*}

\ResultsFigWithHeaderWithZoom{\bricks}{denoising_bricks}{0\%}{25\%}{100\%}{\nspp{1}, 1683\%}

\ResultsFigNoHeaderWithZoom{\mandelbrot}{denoising_mandelbrot}{0\%}{42\%}{100\%}{\nspp{3}, 2255\%}

\ResultsFigNoHeaderWithZoom{\mandelbulb}{denoising_mandelbulb}{0\%}{64\%}{100\%}{\nspp{3}, 600\%}

%\ResultsFigNoHeaderWithZoom{\marble}{denoising_marble}{0\%}{61\%}{100\%}{\nspp{1}, 727\%}

\ResultsFigNoHeaderWithZoom{\marble}{denoising_marble2}{0\%}{61\%}{100\%}{\nspp{1}, 727\%}

\ResultsFigNoHeaderWithZoom{\oceanic}{denoising_oceanic}{0\%}{81\%}{100\%}{\nspp{1}, 1161\%}

\vspace{-2ex}
\caption{\changedh{
Learning to reduce sampling noise in procedural shaders \bricks, \mandelbulb, \marble\ and \oceanic.}
%
The reference low-noise solution (a) relies on 1000 samples per pixel (\spp). Our method (b) approximates the reference well at only \nspp{1}. Zooming into the region boxed in green (c-d) reveals approximation error, which compares favorably with the two baseline methods: (e) RGBx and (f) supersampling, where the number of sample is chosen to have comparable run-time as our method.
%
\changedh{We report relative perceptual error compared with the RGBx baseline (e). Our method better covers both the orientation and high-frequency detail than baseline method.}
}
\label{fig:result_denoising1}
\end{figure*}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig_denoising2.tex <==
\begin{figure*}
    
\ResultsFigWithHeaderWithZoom{\primitives}{denoising_primitives}{0\%}{74\%}{100\%}{\nspp{1}, 1755\%}

\ResultsFigNoHeaderWithZoom{\trippy}{denoising_trippy}{0\%}{74\%}{100\%}{\nspp{4}, 311\%}

\ResultsFigNoHeaderWithZoom{\venice}{denoising_venice}{0\%}{81\%}{100\%}{\nspp{1}, 927\%}

\vspace{-2ex}
\caption{\changedh{Denoising result for shaders \primitives, \trippy\ and \venice. Relative perceptual error reported below each image as in \fig{fig:result_denoising1}.} 
%
For \primitives, our method better recovers the orientation and high-frequency detail of the 3D geometry. For \trippy, our method better reproduces high-frequency texture.
}
\label{fig:result_denoising2}
\end{figure*}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig_post_processing.tex <==
\begin{figure*}

   \ResultsFigWithHeaderThreeCol{\mandelbulb\ blur: 0\%/1x}{new_submission/post_processing_mandelbulb_blur}{100\%/700x (baseline)}{65\%/590x}
    
    \ResultsFigNoHeaderThreeCol{\trippy\ simplified\ sharpen: 0\%/1x}{new_submission/post_processing_trippy_simplified_sharpen}{100\%/340x (baseline)}{80\%/270x}
    
\vspace{-2ex}
\caption{Learning postprocessing effects. The reference solution (a) shows the result of a postprocessing filter applied to a low-noise shader rendering sampled at \nspp{1000}. Both RGBx baseline (b) and our method (c) approximates the reference at \nspp{1}. Our method recovers more faithfully the thin structure in \mandelbulb\ and the color pattern in \trippy. We report relative perceptual error \changedi{and speedup} as in \fig{fig:teaser}. \changedi{\mandelbulb\ is gamma corrected so it can be viewed comfortably on darker displays.}}
\label{fig:result_fig_post_processing}
\end{figure*}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig_simplified.tex <==
\begin{figure*}

    \ResultsFigWithHeaderInputWithZoom{\mandelbrot}{new_submission/simplified_mandelbrot}{0\%/1x}{38\%/1300x}{100\%/1500x}{4.4x/2400x}
    
    \ResultsFigNoHeaderInputWithZoom{\mandelbulb}{new_submission/simplified_mandelbulb}{0\%/1x}{64\%/920x}{100\%/1100x}{2.9x/1800x}
    
    \ResultsFigNoHeaderInputWithZoom{\trippy}{new_submission/simplified_trippy}{0\%/1x}{75\%/270x}{100\%/340x}{2.8x/1600x}
    
\vspace{-2ex}
\caption{\changedi{Learning from simplified shaders \mandelbrot, \mandelbulb\ and \trippy. Errors and speedups are reported as in \fig{fig:teaser}. In \mandelbrot\ our method better reconstructs missing regions due to oversimplification in the input. In \mandelbulb\ our method better recovers the orientation of the texture. In \trippy\ ours correctly recovers the color.}}
\label{fig:result_simplified}

\vspace*{-1.0\baselineskip}

\end{figure*}

==> Learning from Shader Program Traces (EG format)/figtex/result_fig_temporal.tex <==
\begin{figure}[b!]
\centering
\setlength{\h}{1.6in}
    \centering
    \begin{tabular}{cc}
(a) RGBx Baseline & (b) Our result \\
\includegraphics[width=\h]{result_figs/new_submission/trippy_simplified_temporal_RGBx.png} & \includegraphics[width=\h]{result_figs/new_submission/trippy_simplified_temporal_ours.png} \\
\small{\trippy: 100\%} & \small{\changedi{77}\%} \\
\end{tabular}
    \caption{Learning temporally coherent sequences for \trippy\ with the same ground truth as in \fig{fig:result_simplified}. We report relative perceptual error compared to the RGBx baseline. Both RGBx (a) and ours (b) are the 90th frame of a synthesized temporally coherent sequence. Note how our method generalizes well to long sequences whereas the RGBx baseline presents obvious artifacts \changedi{such as color residual from previous frames near the silhouette of the heart.}}
    \label{fig:result_temporal}
\end{figure}

==> Learning from Shader Program Traces (EG format)/figtex/result_pool.tex <==

    
    \vspace{-1ex}
    \setlength{\tabcolsep}{4.0pt}
    \begin{table}[]
    \begin{tabular}{l|r@{}l@{ / }r@{}lr@{\%}l@{ / }r@{\%}l}
    \hline

        Shader & \multicolumn{4}{c}{RGBx} & \multicolumn{4}{c}{Ours} \\ \thickhline
    
         \mandelbrot & 1.3 & e-01 & 7.9 & e-04 & \textbf{05} & & \textbf{25} & \\ \hline
         simp \mandelbrot & 1.6 & e-01 & \textbf{4.6} & \textbf{e-03} & \textbf{56} & & 103 & \\ \hline
         \mandelbulb & 2.4 & e-02 & 8.8 & e-04 & \textbf{49} & & \textbf{52} & \\ \hline
         simp \mandelbulb & 1.4 & e-01 & \textbf{7.1} & \textbf{e-03} & \textbf{77} & & 101 & \\ \hline
         \trippy & 6.1 & e-02 & 2.2 & e-03 & \textbf{78} & & \textbf{81} & \\ \hline
         simp \trippy & 2.4 & e-01 & 1.4 & e-02 & \textbf{70} & & \textbf{56} & \\ \hline
    \end{tabular}
    \caption{temporal}
    \end{table}


    
    
    \begin{figure*}
    
    \ResultsFigNoHeaderWithZoom{\mandelbulb}{new_submission/denoising_mandelbulb}{0\%}{63\%}{100\% (baseline)}{2\,SPP, 8.5x}
    
    \vspace{-2ex}
    \caption{denoising}
    \end{figure*}

    \begin{figure*}
    
    \ResultsFigWithHeaderWithZoom{\trippy}{new_submission/denoising_trippy}{0\%}{78\%}{100\% (baseline)}{9\,SPP, 1.8x}
    
    \ResultsFigNoHeaderWithZoom{\venice}{new_submission/denoising_venice}{0\%}{79\%}{100\% (baseline)}{1\,SPP, 9.3x}
    
    \vspace{-2ex}
    \caption{denoising}
    \end{figure*}
    
    \begin{figure*}
    
    \ResultsFigWithHeaderWithoutZoom{\bricks: 0\%}{new_submission/simplified_bricks}{63\%}{100\% (baseline)}{5.4x}
    
    \vspace{-2ex}
    \caption{simplified}
    \end{figure*}
    
    \begin{figure*}
    
    \ResultsFigWithHeaderThreeCol{\mandelbulb\ blur: 0\%}{new_submission/post_processing_mandelbulb_blur}{100\% (baseline)}{65\%}
    
    \ResultsFigNoHeaderThreeCol{\trippy\ sharpen: 0\%}{new_submission/post_processing_trippy_sharpen}{100\% (baseline)}{78\%}
    
    \ResultsFigNoHeaderThreeCol{\trippy\ simplified\ sharpen: 0\%}{new_submission/post_processing_trippy_simplified_sharpen}{100\% (baseline)}{80\%}
    
    \vspace{-2ex}
    \caption{post processing}
    \end{figure*}
    

    
    

==> Learning from Shader Program Traces (EG format)/figtex/simulation_boids.tex <==
\begin{figure}[b!]
%\vspace{2\baselineskip}
\vspace{-2pt}
\centering
\setlength{\h}{1.17in}
    \centering
    \begin{tabular}{cc}
\includegraphics[height=\h]{result_figs/new_submission/boids_overlap.pdf} & \includegraphics[height=\h]{result_figs/new_submission/boids_metric.png} \\
(a) Visualization & (b) Error Analysis \\
\end{tabular}
\caption{(a) Visualization for flocks of boids. Both I/O baseline (red) and our method (blue) starts from the same initial state and have taken \changedi{80} inference steps with step size 20. Our mean position as well as flocking behavior is more faithful to the ground truth (green). (b) We plot average error as a function of step size, where training ranges from step size 20 to 64 (gray). Ours consistently outperforms both I/O and a more naive baseline, in the training range and beyond it.}

    \label{fig:simulation_boids}
\end{figure}

==> Learning from Shader Program Traces (EG format)/figtex/simulation_fluid.tex <==
\begin{figure}[b!]
\centering
\setlength{\h}{1.05in}
    \centering
    \begin{tabular}{ccc}
(a) Reference & (b) I/O Baseline & (c) Our Method \\
\includegraphics[width=\h]{result_figs/new_submission/fluid_gt.png} & \includegraphics[width=\h]{result_figs/new_submission/fluid_RGBx.png} & \includegraphics[width=\h]{result_figs/new_submission/fluid_ours.png} \\
\small{0\%} & \small{100\%} & \small{96\%} \\
\end{tabular}
\caption{An example of fluid simulation where our method (c) gives a very similar result as the I/O baseline (b). This indicates our method may not be advantageous for simple learning tasks where the baseline is already good enough to reconstruct the reference (a). The relative perceptual error compared to the I/O baseline is reported below each image.}
    \label{fig:simulation_fluid}
\end{figure}

==> Learning from Shader Program Traces (EG format)/figtex/subsample_tradeoff.tex <==
\begin{figure}
    \centering
    \includegraphics[width=3.2in]{result_figs/mandelbrot_subsample.png}
    \caption{Error vs. Time trade-off for models of the \mandelbrot\ shader with varying trace length.
    %
Blue shows perceptual error relative to the RGBx baseline (green).
%
Red shows inference time (including shader program runtime and network inference).
%
Note that error already drops to about half with trace length 25;
%
and that increased overhead is shallow for longer traces.
}
    \label{fig:subsample_tradeoff}
\end{figure}

==> Learning from Shader Program Traces (EG format)/figtex/summary_bar.tex <==
\begin{figure}
    \centering
    \hspace*{-0.1in}\includegraphics[width=3.5in]{result_figs/new_submission/bar_summary_v2.png}
\vspace*{-1.75\baselineskip}
    \caption{\changedj{Four-application summary: {\textbf{denoising}}, reconstruction from {\textbf{simplified}} shaders, learned {\textbf{post}}-processing effects and {\textbf{sim}}ulation.
%    
The vertical axis shows (in every example)} improved perceptual error compared to each applications' strongest baseline:
%
RGBx for denoising, simplified, and post; and I/O for simulation (\sect{sec:eval}). 
%
Hatching directions denote use of simplified shaders and/or temporally coherent models.
}
    \label{fig:summary_bar}
\vspace*{-1.0\baselineskip}
\end{figure}

==> Learning from Shader Program Traces (EG format)/figtex/supp_denoising_table.tex <==

\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}
\begin{table}[]
\begin{tabular}{c|ccccc}
\hline

    \multirow{2}{*}{Shader} &  & \multicolumn{2}{c}{Perceptual} & \multicolumn{2}{c}{L2 Error} \\ \cline{3-6} 
    & Distances: & Similar & Different & Similar & Different \\ \thickhline

    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\bricks\\ Fig1 \end{tabular}}} & RGBx & 6.9e-03 & 2.3e-02 & 9.6e-05 & 2.1e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{28}\% & \textbf{23}\% & \textbf{36}\% & \textbf{28}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 2760\% & 1044\% & 2354\% & 2011\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot\\ Fig1 \end{tabular}}} & RGBx & 8.2e-03 & 9.2e-03 & 2.5e-04 & 2.3e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{40}\% & \textbf{46}\% & \textbf{54}\% & \textbf{64}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 2460\% & 1890\% & 1238\% & 1129\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb\\ Fig1 \end{tabular}}} & RGBx & 8.3e-03 & 9.5e-03 & 3.1e-04 & 2.7e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{64}\% & \textbf{64}\% & \textbf{65}\% & \textbf{70}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 585\% & 627\% & 295\% & 362\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\marble\\ Fig1 \end{tabular}}} & RGBx & 3.1e-02 & 4.4e-02 & 1.4e-03 & 1.7e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{61}\% & \textbf{61}\% & \textbf{53}\% & \textbf{50}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 775\% & 660\% & 1231\% & 1389\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\oceanic\\ Fig1 \end{tabular}}} & RGBx & 3.5e-02 & 4.1e-02 & 4.3e-04 & 4.4e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{83}\% & \textbf{79}\% & \textbf{78}\% & \textbf{81}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 1190\% & 1111\% & 971\% & 1047\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\primitives\\ Fig1 \end{tabular}}} & RGBx & 1.5e-02 & 1.3e-02 & 9.3e-05 & 8.3e-05 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{75}\% & \textbf{72}\% & \textbf{89}\% & \textbf{85}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 1725\% & 1821\% & 1781\% & 2041\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\trippy\\ Fig1 \end{tabular}}} & RGBx & 7.3e-02 & 6.6e-02 & 2.4e-03 & 2.4e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{70}\% & \textbf{81}\% & \textbf{73}\% & \textbf{79}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 316\% & 301\% & 254\% & 241\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\venice\\ Fig1 \end{tabular}}} & RGBx & 3.1e-02 & 2.9e-02 & 6.0e-04 & 5.4e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{80}\% & \textbf{83}\% & \textbf{77}\% & \textbf{79}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 921\% & 940\% & 754\% & 738\% \\ \hline
\end{tabular}
\caption{denoising}
\end{table}

\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}
\begin{table}[]
\begin{tabular}{c|ccccc}
\hline

    \multirow{2}{*}{Shader} &  & \multicolumn{2}{c}{Perceptual} & \multicolumn{2}{c}{L2 Error} \\ \cline{3-6} 
    & Distances: & Similar & Different & Similar & Different \\ \thickhline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\bricks \end{tabular}}} & RGBx & 2.4e-02 & 4.9e-02 & 7.6e-04 & 8.3e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{37}\% & \textbf{41}\% & \textbf{29}\% & \textbf{53}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot \end{tabular}}} & RGBx & 2.2e-01 & 2.9e-01 & 9.9e-03 & 1.7e-02 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{23}\% & \textbf{17}\% & \textbf{24}\% & \textbf{10}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb \end{tabular}}} & RGBx & 8.0e-02 & 5.3e-02 & 5.6e-03 & 2.5e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{56}\% & \textbf{43}\% & \textbf{59}\% & \textbf{43}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\trippy \end{tabular}}} & RGBx & 2.2e-01 & 2.9e-01 & 1.3e-02 & 2.0e-02 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{65}\% & \textbf{71}\% & \textbf{57}\% & \textbf{49}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\venice \end{tabular}}} & RGBx & 4.3e-02 & 4.0e-02 & 9.3e-04 & 8.3e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{78}\% & \textbf{83}\% & \textbf{77}\% & \textbf{81}\% \\ \hline
\end{tabular}
\caption{simplified}
\end{table}

\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}
\begin{table}[]
\begin{tabular}{c|ccccc}
\hline

    \multirow{2}{*}{Shader} &  & \multicolumn{2}{c}{Perceptual} & \multicolumn{2}{c}{L2 Error} \\ \cline{3-6} 
    & Distances: & Similar & Different & Similar & Different \\ \thickhline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot \end{tabular}}} & RGBx & 3.9e-03 & 6.4e-03 & 1.6e-04 & 1.7e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{81}\% & \textbf{73}\% & \textbf{72}\% & \textbf{85}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot\\simplified \end{tabular}}} & RGBx & 1.7e-01 & 1.1e-01 & 1.2e-02 & 6.5e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{36}\% & \textbf{38}\% & \textbf{23}\% & \textbf{27}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb \end{tabular}}} & RGBx & 8.0e-03 & 8.2e-03 & 3.2e-04 & 2.8e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{60}\% & \textbf{64}\% & \textbf{58}\% & \textbf{62}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb\\simplified \end{tabular}}} & RGBx & 1.2e-01 & 7.4e-02 & 8.5e-03 & 4.4e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{62}\% & \textbf{57}\% & \textbf{52}\% & \textbf{45}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\trippy\\simplified \end{tabular}}} & RGBx & 2.2e-01 & 3.1e-01 & 1.4e-02 & 2.6e-02 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{59}\% & \textbf{63}\% & \textbf{46}\% & \textbf{49}\% \\ \hline
\end{tabular}
\caption{temporal}
\end{table}

\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}
\begin{table}[]
\begin{tabular}{c|ccccc}
\hline

    \multirow{2}{*}{Shader} &  & \multicolumn{2}{c}{Perceptual} & \multicolumn{2}{c}{L2 Error} \\ \cline{3-6} 
    & Distances: & Similar & Different & Similar & Different \\ \thickhline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb\\blur \end{tabular}}} & RGBx & 6.3e-03 & 6.9e-03 & 2.3e-04 & 1.7e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{64}\% & \textbf{63}\% & \textbf{65}\% & \textbf{71}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\trippy\\sharpen \end{tabular}}} & RGBx & 9.2e-02 & 8.6e-02 & 4.0e-03 & 3.8e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{69}\% & \textbf{82}\% & \textbf{70}\% & \textbf{80}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\trippy\\simplified\ sharpen \end{tabular}}} & RGBx & 2.4e-01 & 3.1e-01 & 1.6e-02 & 2.5e-02 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{74}\% & \textbf{80}\% & \textbf{62}\% & \textbf{57}\% \\ \hline
\end{tabular}
\caption{post\ processing}
\end{table}


==> Learning from Shader Program Traces (EG format)/figtex/teaser.tex <==
\teaser{
\vspace{-2\baselineskip}    
\ResultsFigTeaser{\venice: 1x speedup, 0\% error}{new_submission/teaser_simplified_venice}{1400x speedup, 7.4x error}{1300x speedup, 100\% error (baseline)}{1300x speedup, 70\% error}
%\vspace{-1\baselineskip}
  \caption{Learning to extrapolate from the partial computation of a procedural shader called \venice. The reference solution (a) results from a full computation at \changedi{1000} samples per pixel (\spp). A simplified version of the shader provides an approximate solution (b) using only \nspp{1} and less computation per sample (\changedi{72}\% of the original compute; \changedi{1400}x speedup overall). Our RGBx baseline method (c) learns to approximate the reference well for much of the image, based on only the RGB output of the simplified shader as well as a few hand-picked auxiliary features~-- but exhibits artifacts in the distance (obvious in the zooms boxed in green). This paper shows that difficult learning tasks like this can benefit from relying on not just the RGBx features but also the \emph{program trace} (a record of the intermediate values computed at every pixel, in this case that of the simplified shader) -- producing a more faithful approximation of the reference. Percent (\%) denotes mean perceptual error~\cite{zhang2018perceptual} relative to that of the RGBx baseline, averaged over the test set.}
\vspace{2ex}
\label{fig:teaser}
}

==> Learning from Shader Program Traces (EG format)/figtex/tiles.tex <==
\begin{figure}
\setlength{\w}{0.52in}
\setlength{\tabcolsep}{1.5pt}
    \centering
    \begin{tabular}{cccccc}
\includegraphics[width=\w]{results/tile_low_saliency1.png} & \includegraphics[width=\w]{results/tile_low_saliency2.png} & \includegraphics[width=\w]{results/tile_medium_saliency1.png} &
\includegraphics[width=\w]{results/tile_medium_saliency2.png} &
\includegraphics[width=\w]{results/tile_high_saliency1.png} & 
\includegraphics[width=\w]{results/tile_high_saliency2.png} \\
\includegraphics[width=\w]{results/tile_low_saliency3.png} & \includegraphics[width=\w]{results/tile_low_saliency4.png} & \includegraphics[width=\w]{results/tile_medium_saliency3.png} &
\includegraphics[width=\w]{results/tile_medium_saliency4.png} &
\includegraphics[width=\w]{results/tile_high_saliency3.png} & 
\includegraphics[width=\w]{results/tile_high_saliency4.png} \\
\multicolumn{2}{c}{(a) sky: low saliency} & \multicolumn{2}{c}{(b) waves: medium} & \multicolumn{2}{c}{(c) sun: high saliency}\\
\end{tabular}
    \caption{Manual identification of saliency for tile clusters from \oceanic. Groups of four tiles selected randomly from 
    clusters, arranged by saliency.}
    \label{fig:tiles}
\end{figure}


==> Learning from Shader Program Traces (EG format)/figtex/trace_subsample_comparison.tex <==
\begin{figure}
    \centering
    %\includegraphics[width=3.3in]{result_figs/new_submission/trace_subsample_comparison.png}
    \includegraphics[width=3.3in]{result_figs/new_submission/fig5.pdf}
    \caption{\changedi{Error vs. Time trade-off for Opponent, Uniform, and Oracle subsampling strategies with varying trace length. For each shader with \trace\ program traces, we subsample the trace such that the actual input trace length \tracelen\ is equal to \trace/2, \trace/4, \trace/8, etc., and the x-axis shows each model's relative trace ratio compared to the full program trace. Circle shows perceptual error relative to the RGBx baseline (green square) for Opponent (red), Uniform (purple), Oracle (blue), and Full Trace (gold). Black pentagon shows relative inference time (including shader program runtime and network inference) for each \tracelen\ relative to the runtime of the Full Trace model. Similarly black square shows relative inference time for the RGBx baseline. Note that the x-axis is on a log scale in relative trace length compared to the Full Trace model, therefore although the relative error plot appears linear as \tracelen\ increases, the actual performance improvement is faster at the beginning of the plot: adding only a few traces quickly improves performance.}}

    \label{fig:trace_subsample_comparison}
\end{figure}

==> Learning from Shader Program Traces (EG format)/figtex/visualize_channels.tex <==
\begin{figure}[b!]
\centering
\setlength{\w}{1.55in}
%\setlength{\tabcolsep}{1.5pt}
    \centering
    \begin{tabular}{cc}
\includegraphics[width=\w]{result_figs/new_submission/visualize_bricks.png} & \includegraphics[width=\w]{result_figs/new_submission/visualize_mandelbrot.png} \\
(a) \bricks & (b) \mandelbrot \\
\end{tabular}
    \caption{The sorted importance score for each trace feature from two shader programs. The y axis has a log scale \changedi{with higher score indicating the feature is more important.} Each bar in the plot represents a trace from the program. Note that in both shaders, only a few trace elements have high importance.}
    \label{fig:visualize}
\end{figure}

==> a0-description.tex <==
\begin{center}
{\LARGE Appendices} \\ \vspace{0.5\baselineskip}
{\Large \textit{Learning from Shader Program Traces}} \\ \vspace{0.5\baselineskip}
(in review for Eurographics 2022)
\end{center}

\emph{Note to reviewers:} Here we include as appendices some details we removed from the main body of the paper to reduce overall length. Any or all them could be included or omitted as needed.

==> figtex/error-table-data.tex <==
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Shader}} & \multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{2}{c}{Perceptual (\%)} & \multicolumn{2}{c}{L2 Error (\%)} \\ \cline{3-6}
\multicolumn{1}{c|}{} & Distances: & Similar & Different & Similar & Different  \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\oceanic \\ Fig. 1 \\ \tracelen\ = 702\end{tabular}}} & Ours & \textbf{2.85} & \textbf{3.19} & \textbf{1.83} & \textbf{1.86} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 3.34 & 3.72 & 2.04 & 2.05 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 41.62 & 45.23 & 6.46 & 6.75 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\bricks \\ Fig. 2 \\ \tracelen\ = 56\end{tabular}}} & Ours & \textbf{0.23} & \textbf{0.66} & \textbf{0.61} & \textbf{0.83} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 0.66 & 2.43 & 0.97 & 1.45 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 19.12 & 24.34 & 4.75 & 6.55 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb \\ Fig. 2 \\ \tracelen\ = 232\end{tabular}}} & Ours & \textbf{0.51} & \textbf{0.62} & \textbf{1.41} & \textbf{1.40} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 0.81 & 0.93 & 1.76 & 1.65 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 4.84 & 5.92 & 3.04 & 3.15 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\marble \\ Fig. 2 \\ \tracelen\ = 226\end{tabular}}} & Ours & \textbf{1.96} & \textbf{2.68} & \textbf{2.75} & \textbf{2.97} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 3.28 & 5.22 & 3.69 & 3.93 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 23.92 & 28.96 & 13.34 & 15.59 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\texturemap \\ Fig. 2 \\ \tracelen\ = 80\end{tabular}}} & Ours & \textbf{2.15} & \textbf{6.19} & \textbf{1.66} & \textbf{2.31} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 2.86 & 6.77 & 1.88 & 2.42 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 29.77 & 34.77 & 6.12 & 7.81 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\primitives \\ Fig. 5 \\ \tracelen\ = 771\end{tabular}}} & Ours & \textbf{0.96} & \textbf{0.94} & \textbf{1.05} & \textbf{1.06} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 1.23 & 1.17 & 1.10 & 1.11 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 15.37 & 16.24 & 3.26 & 3.28 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\trippy \\ Fig. 5 \\ \tracelen\ = 199\end{tabular}}} & Ours & \textbf{5.37} & \textbf{5.54} & \textbf{4.35} & \textbf{4.44} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 7.17 & 6.50 & 4.91 & 4.84 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 23.13 & 19.91 & 7.84 & 7.54 \\ \thickhline

\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot \\ Fig. 5 \\ \tracelen\ = 131\end{tabular}}} & Ours & \textbf{0.31} & \textbf{0.35} & \textbf{1.17} & \textbf{1.15} \\ \cline{2-6}
\multicolumn{1}{c|}{}& RGB+Aux & 0.83 & 1.07 & 1.55 & 1.51 \\ \cline{2-6}
\multicolumn{1}{c|}{}& Supersample & 23.40 & 19.95 & 6.79 & 6.22 \\ \hline

\end{tabular}

==> figtex/error-table-new.tex <==
\begin{table}
\centering
\caption{Error statistics for shaders in Figures \ref{fig:teaser}, \ref{fig:result_fig1} and \ref{fig:result_fig2}. We report errors for test datasets with similar and different distances to the geometry: see \sect{sec:dataset} for  details. Note that elsewhere in the paper, we simply report a single mean error over the test set. For each test dataset, we report metrics for mean RGB $L^2$ error and perceptual error \cite{zhang2018perceptual}.}
\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}

\input{figtex/error-table-data}

\label{tab:error_breakdown}
\vspace{-2ex}
\end{table}

==> figtex/error_table_post_processing.tex <==
\setlength{\tabcolsep}{4.0pt}
\begin{table}[]
\caption{Errors learning postprocessing filters, as in \tbl{tab:error_denoising}. \changedi{Each postprocessing filter is trained with a specific shader: blur (\mandelbulb), sharpen (\trippy) and simplified sharpen (\trippy).}}
\vspace{-0.75\baselineskip}
\begin{tabular}{l|r@{}l@{ / }r@{}lr@{\%}l@{ / }r@{\%}l}
    \hline

        Shader & \multicolumn{4}{c}{RGBx} & \multicolumn{4}{c}{Ours} \\ \thickhline
    
         blur & 1.2 & e-02 & 3.6 & e-04 & \textbf{65} & & \textbf{69} & \\ \hline
         sharpen & 8.8 & e-02 & 3.8 & e-03 & \textbf{78} & & \textbf{78} & \\ \hline
         simp sharpen & 2.7 & e-01 & 2.0 & e-02 & \textbf{80} & & \textbf{60} & \\ \hline
    \end{tabular}
\label{tab:error_post_processing}
\end{table}

==> figtex/error_table_simplified.tex <==
\vspace{-1ex}
\setlength{\tabcolsep}{4.0pt}
\begin{table}[]
\caption{Errors reconstructing simplified shaders, as in \tbl{tab:error_denoising}.}
\vspace{-0.75\baselineskip}
\begin{tabular}{l|r@{}l@{ / }r@{}lr@{\%}l@{ / }r@{\%}l}
    \hline

        Shader & \multicolumn{4}{c}{RGBx} & \multicolumn{4}{c}{Ours} \\ \thickhline
    
         \bricks & 6.3 & e-02 & 3.0 & e-03 & \textbf{63} & & \textbf{46} & \\ \hline
         \mandelbrot & 1.1 & e-01 & 3.7 & e-03 & \textbf{38} & & \textbf{45} & \\ \hline
         \mandelbulb & 9.3 & e-02 & 5.4 & e-03 & \textbf{64} & & \textbf{72} & \\ \hline
         \trippy & 2.4 & e-01 & 1.5 & e-02 & \textbf{75} & & \textbf{57} & \\ \hline
         \venice & 4.0 & e-02 & 7.2 & e-04 & \textbf{70} & & \textbf{74} & \\ \hline
    \end{tabular}
\label{tab:error_simplified}
\end{table}

==> figtex/error_table_unified.tex <==
\vspace{-1ex}
\setlength{\tabcolsep}{4.0pt}
\begin{table}[]
\caption{\changedi{Errors training a shared denoiser for \mandelbrot, \mandelbulb, \primitives\ and \trippy, as in \tbl{tab:error_denoising}.}}
\vspace{-0.75\baselineskip}
\begin{tabular}{l|r@{}l@{ / }r@{}lr@{\%}l@{ / }r@{\%}l}
    \hline

        Shader & \multicolumn{4}{c}{RGBx} & \multicolumn{4}{c}{Ours} \\ \thickhline
    
         \mandelbrot & 5.4 & e-02 & 1.9 & e-03 & \textbf{30} & & \textbf{35} & \\ \hline
         \mandelbulb & 4.3 & e-02 & 2.0 & e-03 & \textbf{70} & & \textbf{59} & \\ \hline
         \primitives & 2.5 & e-02 & 1.7 & e-04 & \textbf{69} & & \textbf{85} & \\ \hline
         \trippy & 1.0 & e-01 & 1.1 & e-02 & \textbf{72} & & \textbf{40} & \\ \hline
\end{tabular}
\label{tab:error_unified}
\end{table}

==> figtex/mandelbrot_ablation.tex <==
\begin{figure*}
  \setlength{\tabcolsep}{1pt}
  \setlength{\h}{1.14in}
  \vspace{3\baselineskip}
  \begin{tabular}{cccccccc}
  
(a) L2 & (b) Perceptual & (c) All & (d) Every 4th & (e) First 5 & (f) Last 5 & (g) Subsample 4 & (h) Mean \& Var \\
\addlinespace[4pt]
  
 \includegraphics[height=\h]{results/mandelbrot_l2_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_perceptual_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_all_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_every_4th_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_first_5_no_last_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_last_5_zoom_thin.png} & \includegraphics[height=\h]{results/mandelbrot_subsample_4_zoom_thin.png} &  \includegraphics[height=\h]{results/mandelbrot_mean_var_zoom_thin.png} \tablegap

 
{\small 189 ms, 0.65\%} & 
{\small 201 ms, 0.33\%} & 
{\small 265 ms, 0.29\%} &
{\small 226 ms, 0.33\%} & 
{\small 193 ms, 0.35\%} & 
{\small 196 ms, 0.40\%} &
{\small 200 ms, 0.39\%} &
{\small 212 ms, 0.38\%} \\
  
  \end{tabular}
  \vspace{-2ex}
  \caption{Ablation study for shader \mandelbrot. We show our method, with the same zoom regions as in \fig{fig:result_fig2}. Time and error values are reported below each image as in Figure 1. We train a total of 400 epochs for each experiment. In (a-b) we report ablations on the training loss selection, where \mandelbrot's loop is handled the same as in \fig{fig:result_fig2}. (a) L2 loss only; (b) Perceptual loss only. The errors in (a-b) are higher, and thin line structures are broken or blurred. Thus, our method of combining both L2 and perceptual loss is the best. In (c-h) we show the different options for handling loops mentioned in \sect{sec:loops}: we handle the loop by unrolling (c) or sample every 4th trace from the entire program (d), or add to the trace only the first (e) or last (f) 5 iterations of the loop, subsample every 4 iterations (g) or collect mean and variance statistics from all loop iterations (h). (c) is slower than (d-h) because a longer trace must be gathered. (d-h) are slightly visually and quantitatively worse than using all loop iterations (c), but much faster. For comparison, the \mandelbrot\ shader that we selected in \fig{fig:result_fig2} uses the first 5 and last 1 loop iterations: this gives a slightly better visual and quantitative result in a similar running time.}
  \label{fig:mandelbrot_ablation}
\end{figure*}

==> figtex/postprocessing.tex <==
\begin{figure}
\centering
\setlength{\h}{1.5in}
    \centering
    \begin{tabular}{cc}
(a) Ground Truth & (b) Our result \\
\includegraphics[width=\h]{results/postprocessing_defocus_blur_gt.png} & \includegraphics[width=\h]{results/postprocessing_defocus_blur_ours.png} \\
\small{\mandelbulb: defocus} & \small{Perceptual: 0.4\%, L2: 1.2\%} \\ \\
\includegraphics[width=\h]{results/postprocessing_sharpen_gt.png} & \includegraphics[width=\h]{results/postprocessing_sharpen_ours.png} \\
\small{\trippy: sharpen} & \small{Perceptual: 6.9\%, L2: 5.5\%}
\end{tabular}
    \caption{Result images for postprocessing filters: defocus for \mandelbulb\ and sharpen for \trippy. Under our result we report both perceptual and L2 error over the test set.}
    \label{fig:postprocessing}
\end{figure}

==> figtex/result_fig1.tex <==
\begin{figure*}
\ResultsFigWithHeader{\bricks}{bricks}{688 sec}{751 ms, 0.4}{754 ms, 1.3}{\nspp{1}, 688\,ms, 21}
\ResultsFigNoHeader{\mandelbulb}{mandelbulb}{47 sec}{143 ms, 0.5}{115 ms, 0.8}{\nspp{3}, 141\,ms, 5}
\ResultsFigNoHeader{\marble}{marble2}{714 sec}{785 ms, 2.2}{747 ms, 3.9}{\nspp{1}, 714\,ms, 26}
\ResultsFigNoHeader{\texturemap}{texture_map3}{1111 sec}{1177 ms, 3.5}{1165 ms sec, 4.2}{\nspp{1}, 1111\,ms, 31}
  \vspace{-2ex}
  \caption{Denoising shaders \bricks, \mandelbulb, \marble\ and \texturemap. Time and error values are as in Figure 1. Our method better recovers both the orientation and high-frequency detail than the baseline methods.} 
  \label{fig:result_fig1}
  \vspace{-1ex}
\end{figure*}

==> figtex/result_fig2.tex <==
\begin{figure*}
\ResultsFigWithHeader{\primitives}{primitives}{1123 sec}{1325 ms, 1.0}{1217 ms, 1.2}{\nspp{1}, 1123\,ms, 16}
\ResultsFigNoHeader{\trippy}{trippy}{30 sec}{123 ms, 5.4}{97.6 ms, 6.9}{\nspp{4}, 121\,ms, 22}
\ResultsFigNoHeader{\mandelbrot}{mandelbrot}{106 sec}{202 ms, 0.32}{185 ms, 0.91}{\nspp{2}, 212\,ms, 22}
  \vspace{-2ex}
  \caption{Result images for shaders \primitives, \trippy, and \mandelbrot. Time and error values are reported below each image as in Figure 1. For \primitives, our method better recovers the orientation and high-frequency detail of the 3D geometry. For \trippy, our method better reproduces high-frequency texture. For \mandelbrot, our method better preserves thin line structures.}
  \label{fig:result_fig2}
\end{figure*}

==> figtex/result_fig_denoising1.tex <==
\begin{figure*}

\ResultsFigWithHeaderWithZoom{\bricks}{denoising_bricks}{0\%}{25\%}{100\%}{\nspp{1}, 1683\%}

\ResultsFigNoHeaderWithZoom{\mandelbrot}{denoising_mandelbrot}{0\%}{42\%}{100\%}{\nspp{3}, 2255\%}

\ResultsFigNoHeaderWithZoom{\mandelbulb}{denoising_mandelbulb}{0\%}{64\%}{100\%}{\nspp{3}, 600\%}

%\ResultsFigNoHeaderWithZoom{\marble}{denoising_marble}{0\%}{61\%}{100\%}{\nspp{1}, 727\%}

\ResultsFigNoHeaderWithZoom{\marble}{denoising_marble2}{0\%}{61\%}{100\%}{\nspp{1}, 727\%}

\ResultsFigNoHeaderWithZoom{\oceanic}{denoising_oceanic}{0\%}{81\%}{100\%}{\nspp{1}, 1161\%}

\vspace{-2ex}
\caption{\changedh{
Learning to reduce sampling noise in procedural shaders \bricks, \mandelbulb, \marble\ and \oceanic.}
%
The reference low-noise solution (a) relies on 1000 samples per pixel (\spp). Our method (b) approximates the reference well at only \nspp{1}. Zooming into the region boxed in green (c-d) reveals approximation error, which compares favorably with the two baseline methods: (e) RGBx and (f) supersampling, where the number of sample is chosen to have comparable run-time as our method.
%
\changedh{We report relative perceptual error compared with the RGBx baseline (e). Our method better covers both the orientation and high-frequency detail than baseline method.}
}
\label{fig:result_denoising1}
\end{figure*}

==> figtex/result_fig_denoising2.tex <==
\begin{figure*}
    
\ResultsFigWithHeaderWithZoom{\primitives}{denoising_primitives}{0\%}{74\%}{100\%}{\nspp{1}, 1755\%}

\ResultsFigNoHeaderWithZoom{\trippy}{denoising_trippy}{0\%}{74\%}{100\%}{\nspp{4}, 311\%}

\ResultsFigNoHeaderWithZoom{\venice}{denoising_venice}{0\%}{81\%}{100\%}{\nspp{1}, 927\%}

\vspace{-2ex}
\caption{\changedh{Denoising result for shaders \primitives, \trippy\ and \venice. Relative perceptual error reported below each image as in \fig{fig:result_denoising1}.} 
%
For \primitives, our method better recovers the orientation and high-frequency detail of the 3D geometry. For \trippy, our method better reproduces high-frequency texture.
}
\label{fig:result_denoising2}
\end{figure*}

==> figtex/result_pool.tex <==

    
    \vspace{-1ex}
    \setlength{\tabcolsep}{4.0pt}
    \begin{table}[]
    \begin{tabular}{l|r@{}l@{ / }r@{}lr@{\%}l@{ / }r@{\%}l}
    \hline

        Shader & \multicolumn{4}{c}{RGBx} & \multicolumn{4}{c}{Ours} \\ \thickhline
    
         \mandelbrot & 1.3 & e-01 & 7.9 & e-04 & \textbf{05} & & \textbf{25} & \\ \hline
         simp \mandelbrot & 1.6 & e-01 & \textbf{4.6} & \textbf{e-03} & \textbf{56} & & 103 & \\ \hline
         \mandelbulb & 2.4 & e-02 & 8.8 & e-04 & \textbf{49} & & \textbf{52} & \\ \hline
         simp \mandelbulb & 1.4 & e-01 & \textbf{7.1} & \textbf{e-03} & \textbf{77} & & 101 & \\ \hline
         \trippy & 6.1 & e-02 & 2.2 & e-03 & \textbf{78} & & \textbf{81} & \\ \hline
         simp \trippy & 2.4 & e-01 & 1.4 & e-02 & \textbf{70} & & \textbf{56} & \\ \hline
    \end{tabular}
    \caption{temporal}
    \end{table}


    
    
    \begin{figure*}
    
    \ResultsFigNoHeaderWithZoom{\mandelbulb}{new_submission/denoising_mandelbulb}{0\%}{63\%}{100\% (baseline)}{2\,SPP, 8.5x}
    
    \vspace{-2ex}
    \caption{denoising}
    \end{figure*}

    \begin{figure*}
    
    \ResultsFigWithHeaderWithZoom{\trippy}{new_submission/denoising_trippy}{0\%}{78\%}{100\% (baseline)}{9\,SPP, 1.8x}
    
    \ResultsFigNoHeaderWithZoom{\venice}{new_submission/denoising_venice}{0\%}{79\%}{100\% (baseline)}{1\,SPP, 9.3x}
    
    \vspace{-2ex}
    \caption{denoising}
    \end{figure*}
    
    \begin{figure*}
    
    \ResultsFigWithHeaderWithoutZoom{\bricks: 0\%}{new_submission/simplified_bricks}{63\%}{100\% (baseline)}{5.4x}
    
    \vspace{-2ex}
    \caption{simplified}
    \end{figure*}
    
    \begin{figure*}
    
    \ResultsFigWithHeaderThreeCol{\mandelbulb\ blur: 0\%}{new_submission/post_processing_mandelbulb_blur}{100\% (baseline)}{65\%}
    
    \ResultsFigNoHeaderThreeCol{\trippy\ sharpen: 0\%}{new_submission/post_processing_trippy_sharpen}{100\% (baseline)}{78\%}
    
    \ResultsFigNoHeaderThreeCol{\trippy\ simplified\ sharpen: 0\%}{new_submission/post_processing_trippy_simplified_sharpen}{100\% (baseline)}{80\%}
    
    \vspace{-2ex}
    \caption{post processing}
    \end{figure*}
    

    
    

==> figtex/subsample_tradeoff.tex <==
\begin{figure}
    \centering
    \includegraphics[width=3.2in]{result_figs/mandelbrot_subsample.png}
    \caption{Error vs. Time trade-off for models of the \mandelbrot\ shader with varying trace length.
    %
Blue shows perceptual error relative to the RGBx baseline (green).
%
Red shows inference time (including shader program runtime and network inference).
%
Note that error already drops to about half with trace length 25;
%
and that increased overhead is shallow for longer traces.
}
    \label{fig:subsample_tradeoff}
\end{figure}

==> figtex/supp_denoising_table.tex <==

\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}
\begin{table}[]
\begin{tabular}{c|ccccc}
\hline

    \multirow{2}{*}{Shader} &  & \multicolumn{2}{c}{Perceptual} & \multicolumn{2}{c}{L2 Error} \\ \cline{3-6} 
    & Distances: & Similar & Different & Similar & Different \\ \thickhline

    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\bricks\\ Fig1 \end{tabular}}} & RGBx & 6.9e-03 & 2.3e-02 & 9.6e-05 & 2.1e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{28}\% & \textbf{23}\% & \textbf{36}\% & \textbf{28}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 2760\% & 1044\% & 2354\% & 2011\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot\\ Fig1 \end{tabular}}} & RGBx & 8.2e-03 & 9.2e-03 & 2.5e-04 & 2.3e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{40}\% & \textbf{46}\% & \textbf{54}\% & \textbf{64}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 2460\% & 1890\% & 1238\% & 1129\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb\\ Fig1 \end{tabular}}} & RGBx & 8.3e-03 & 9.5e-03 & 3.1e-04 & 2.7e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{64}\% & \textbf{64}\% & \textbf{65}\% & \textbf{70}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 585\% & 627\% & 295\% & 362\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\marble\\ Fig1 \end{tabular}}} & RGBx & 3.1e-02 & 4.4e-02 & 1.4e-03 & 1.7e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{61}\% & \textbf{61}\% & \textbf{53}\% & \textbf{50}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 775\% & 660\% & 1231\% & 1389\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\oceanic\\ Fig1 \end{tabular}}} & RGBx & 3.5e-02 & 4.1e-02 & 4.3e-04 & 4.4e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{83}\% & \textbf{79}\% & \textbf{78}\% & \textbf{81}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 1190\% & 1111\% & 971\% & 1047\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\primitives\\ Fig1 \end{tabular}}} & RGBx & 1.5e-02 & 1.3e-02 & 9.3e-05 & 8.3e-05 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{75}\% & \textbf{72}\% & \textbf{89}\% & \textbf{85}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 1725\% & 1821\% & 1781\% & 2041\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\trippy\\ Fig1 \end{tabular}}} & RGBx & 7.3e-02 & 6.6e-02 & 2.4e-03 & 2.4e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{70}\% & \textbf{81}\% & \textbf{73}\% & \textbf{79}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 316\% & 301\% & 254\% & 241\% \\ \thickhline
    \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\venice\\ Fig1 \end{tabular}}} & RGBx & 3.1e-02 & 2.9e-02 & 6.0e-04 & 5.4e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{80}\% & \textbf{83}\% & \textbf{77}\% & \textbf{79}\% \\ \cline{2-6}
    \multicolumn{1}{c|}{} & MSAA & 921\% & 940\% & 754\% & 738\% \\ \hline
\end{tabular}
\caption{denoising}
\end{table}

\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}
\begin{table}[]
\begin{tabular}{c|ccccc}
\hline

    \multirow{2}{*}{Shader} &  & \multicolumn{2}{c}{Perceptual} & \multicolumn{2}{c}{L2 Error} \\ \cline{3-6} 
    & Distances: & Similar & Different & Similar & Different \\ \thickhline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\bricks \end{tabular}}} & RGBx & 2.4e-02 & 4.9e-02 & 7.6e-04 & 8.3e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{37}\% & \textbf{41}\% & \textbf{29}\% & \textbf{53}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot \end{tabular}}} & RGBx & 2.2e-01 & 2.9e-01 & 9.9e-03 & 1.7e-02 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{23}\% & \textbf{17}\% & \textbf{24}\% & \textbf{10}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb \end{tabular}}} & RGBx & 8.0e-02 & 5.3e-02 & 5.6e-03 & 2.5e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{56}\% & \textbf{43}\% & \textbf{59}\% & \textbf{43}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\trippy \end{tabular}}} & RGBx & 2.2e-01 & 2.9e-01 & 1.3e-02 & 2.0e-02 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{65}\% & \textbf{71}\% & \textbf{57}\% & \textbf{49}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\venice \end{tabular}}} & RGBx & 4.3e-02 & 4.0e-02 & 9.3e-04 & 8.3e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{78}\% & \textbf{83}\% & \textbf{77}\% & \textbf{81}\% \\ \hline
\end{tabular}
\caption{simplified}
\end{table}

\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}
\begin{table}[]
\begin{tabular}{c|ccccc}
\hline

    \multirow{2}{*}{Shader} &  & \multicolumn{2}{c}{Perceptual} & \multicolumn{2}{c}{L2 Error} \\ \cline{3-6} 
    & Distances: & Similar & Different & Similar & Different \\ \thickhline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot \end{tabular}}} & RGBx & 3.9e-03 & 6.4e-03 & 1.6e-04 & 1.7e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{81}\% & \textbf{73}\% & \textbf{72}\% & \textbf{85}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbrot\\simplified \end{tabular}}} & RGBx & 1.7e-01 & 1.1e-01 & 1.2e-02 & 6.5e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{36}\% & \textbf{38}\% & \textbf{23}\% & \textbf{27}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb \end{tabular}}} & RGBx & 8.0e-03 & 8.2e-03 & 3.2e-04 & 2.8e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{60}\% & \textbf{64}\% & \textbf{58}\% & \textbf{62}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb\\simplified \end{tabular}}} & RGBx & 1.2e-01 & 7.4e-02 & 8.5e-03 & 4.4e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{62}\% & \textbf{57}\% & \textbf{52}\% & \textbf{45}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\trippy\\simplified \end{tabular}}} & RGBx & 2.2e-01 & 3.1e-01 & 1.4e-02 & 2.6e-02 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{59}\% & \textbf{63}\% & \textbf{46}\% & \textbf{49}\% \\ \hline
\end{tabular}
\caption{temporal}
\end{table}

\vspace{-1ex}
\setlength{\tabcolsep}{2.0pt}
\begin{table}[]
\begin{tabular}{c|ccccc}
\hline

    \multirow{2}{*}{Shader} &  & \multicolumn{2}{c}{Perceptual} & \multicolumn{2}{c}{L2 Error} \\ \cline{3-6} 
    & Distances: & Similar & Different & Similar & Different \\ \thickhline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\mandelbulb\\blur \end{tabular}}} & RGBx & 6.3e-03 & 6.9e-03 & 2.3e-04 & 1.7e-04 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{64}\% & \textbf{63}\% & \textbf{65}\% & \textbf{71}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\trippy\\sharpen \end{tabular}}} & RGBx & 9.2e-02 & 8.6e-02 & 4.0e-03 & 3.8e-03 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{69}\% & \textbf{82}\% & \textbf{70}\% & \textbf{80}\% \\ \thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\trippy\\simplified\ sharpen \end{tabular}}} & RGBx & 2.4e-01 & 3.1e-01 & 1.6e-02 & 2.5e-02 \\ \cline{2-6} 
    \multicolumn{1}{c|}{} & Ours & \textbf{74}\% & \textbf{80}\% & \textbf{62}\% & \textbf{57}\% \\ \hline
\end{tabular}
\caption{post\ processing}
\end{table}


==> figtex/tiles.tex <==
\begin{figure}
\setlength{\w}{0.52in}
\setlength{\tabcolsep}{1.5pt}
    \centering
    \begin{tabular}{cccccc}
\includegraphics[width=\w]{results/tile_low_saliency1.png} & \includegraphics[width=\w]{results/tile_low_saliency2.png} & \includegraphics[width=\w]{results/tile_medium_saliency1.png} &
\includegraphics[width=\w]{results/tile_medium_saliency2.png} &
\includegraphics[width=\w]{results/tile_high_saliency1.png} & 
\includegraphics[width=\w]{results/tile_high_saliency2.png} \\
\includegraphics[width=\w]{results/tile_low_saliency3.png} & \includegraphics[width=\w]{results/tile_low_saliency4.png} & \includegraphics[width=\w]{results/tile_medium_saliency3.png} &
\includegraphics[width=\w]{results/tile_medium_saliency4.png} &
\includegraphics[width=\w]{results/tile_high_saliency3.png} & 
\includegraphics[width=\w]{results/tile_high_saliency4.png} \\
\multicolumn{2}{c}{(a) sky: low saliency} & \multicolumn{2}{c}{(b) waves: medium} & \multicolumn{2}{c}{(c) sun: high saliency}\\
\end{tabular}
    \caption{Manual identification of saliency for tile clusters from \oceanic. Groups of four tiles selected randomly from 
    clusters, arranged by saliency.}
    \label{fig:tiles}
\end{figure}


==> figtex/visualize_channels.tex <==
\begin{figure}[b!]
\centering
\setlength{\w}{1.55in}
%\setlength{\tabcolsep}{1.5pt}
    \centering
    \begin{tabular}{cc}
\includegraphics[width=\w]{result_figs/new_submission/visualize_bricks.png} & \includegraphics[width=\w]{result_figs/new_submission/visualize_mandelbrot.png} \\
(a) \bricks & (b) \mandelbrot \\
\end{tabular}
    \caption{The sorted importance score for each trace feature from two shader programs. The y axis has a log scale \changedi{with higher score indicating the feature is more important.} Each bar in the plot represents a trace from the program. Note that in both shaders, only a few trace elements have high importance.}
    \label{fig:visualize}
\end{figure}
